More Is Never Less: Affordable Robustness to Additive Attacks via Monotone Multiple-Instance Learning

Static malware detectors that represent each sample as a bag of extracted features, such as permissions, API calls, or imported functions, are cheap to deploy and remain state-of-the-art under temporal drift and in selective classification. Yet, attackers can evade them by adding benign-looking content that outweighs malicious evidence. Canonically, detectors encode the presence of a few thousand features, selected during training, as sparse multi-hot vectors over a fixed vocabulary. Features that emerge after training remain invisible. We show that linear models and multi-layer perceptrons (MLPs) over this input are sum-pooled set models in disguise. Sum-pooling lets added benign features cancel malicious evidence. Instead, we cast malware detection with set-shaped static features as a multiple-instance learning (MIL) problem. To this end, we propose MalSets, which uses max-pooled Deep Sets models with a monotone head to ensure that any malicious evidence remains undiluted; thus, more is never less. Under MIL, a general text encoder maps any feature string to an embedding, thus eliminating the long-standing out-of-vocabulary problem at test time. Max-pooling retains the malicious evidence regardless of how many benign features an attacker adds. Since max-pooling can only grow when features are added, constraining the head alone makes the malware score monotone under additions, even against a white-box attacker adapted to this architecture. While monotone detectors are never evaded by state-of-the-art black-box or white-box attacks, they often significantly pay for this robustness in clean performance since benign features cannot count as evidence. However, by combining a non-monotone set encoder with max-pooling and a monotone head, MalSets maintains the robustness of prior monotone classifiers while achieving state-of-the-art performance.

==> figures/polarity_baselines_data/summary.tex <==
\def\polDDmissing{0}
\def\polDDarrows{0.1975/19.57/34.19/polBen,0.4225/5.14/21.47/polBen,0.7375/26.12/11.01/polMal,0.9475/48.38/14.19/polMal}
\def\polDDhasarrows{1}
\def\polDDben{18\,$\to$\,29\,\%}
\def\polDDmal{28\,$\to$\,13\,\%}
\def\polDDsplit{0.52000}
\def\polDDn{109}
\def\polDDev{109}
\def\polDDC{200}
\def\polDDstrip{0.0000/0.0050/polBen!100!white,0.0050/0.0100/polBen!91!white,0.0100/0.0150/polBen!90!white,0.0150/0.0200/polBen!89!white,0.0200/0.0250/polBen!87!white,0.0250/0.0300/polBen!85!white,0.0300/0.0350/polBen!84!white,0.0350/0.0400/polBen!84!white,0.0400/0.0450/polBen!82!white,0.0450/0.0500/polBen!81!white,0.0500/0.0550/polBen!81!white,0.0550/0.0600/polBen!81!white,0.0600/0.0650/polBen!80!white,0.0650/0.0700/polBen!80!white,0.0700/0.0750/polBen!78!white,0.0750/0.0800/polBen!78!white,0.0800/0.0850/polBen!77!white,0.0850/0.0900/polBen!77!white,0.0900/0.0950/polBen!76!white,0.0950/0.1000/polBen!75!white,0.1000/0.1050/polBen!75!white,0.1050/0.1100/polBen!73!white,0.1100/0.1150/polBen!73!white,0.1150/0.1200/polBen!72!white,0.1200/0.1250/polBen!72!white,0.1250/0.1300/polBen!70!white,0.1300/0.1350/polBen!70!white,0.1350/0.1400/polBen!68!white,0.1400/0.1450/polBen!67!white,0.1450/0.1500/polBen!67!white,0.1500/0.1550/polBen!64!white,0.1550/0.1600/polBen!63!white,0.1600/0.1650/polBen!63!white,0.1650/0.1700/polBen!62!white,0.1700/0.1750/polBen!62!white,0.1750/0.1800/polBen!60!white,0.1800/0.1850/polBen!59!white,0.1850/0.1900/polBen!59!white,0.1900/0.1950/polBen!59!white,0.1950/0.2000/polBen!59!white,0.2000/0.2050/polBen!58!white,0.2050/0.2100/polBen!58!white,0.2100/0.2150/polBen!56!white,0.2150/0.2200/polBen!55!white,0.2200/0.2250/polBen!55!white,0.2250/0.2300/polBen!53!white,0.2300/0.2350/polBen!53!white,0.2350/0.2400/polBen!53!white,0.2400/0.2450/polBen!53!white,0.2450/0.2500/polBen!52!white,0.2500/0.2550/polBen!52!white,0.2550/0.2600/polBen!50!white,0.2600/0.2650/polBen!50!white,0.2650/0.2700/polBen!49!white,0.2700/0.2750/polBen!49!white,0.2750/0.2800/polBen!47!white,0.2800/0.2850/polBen!47!white,0.2850/0.2900/polBen!47!white,0.2900/0.2950/polBen!47!white,0.2950/0.3000/polBen!47!white,0.3000/0.3050/polBen!45!white,0.3050/0.3100/polBen!44!white,0.3100/0.3150/polBen!44!white,0.3150/0.3200/polBen!44!white,0.3200/0.3250/polBen!42!white,0.3250/0.3300/polBen!42!white,0.3300/0.3350/polBen!42!white,0.3350/0.3400/polBen!40!white,0.3400/0.3450/polBen!40!white,0.3450/0.3500/polBen!38!white,0.3500/0.3550/polBen!38!white,0.3550/0.3600/polBen!38!white,0.3600/0.3650/polBen!38!white,0.3650/0.3700/polBen!38!white,0.3700/0.3750/polBen!36!white,0.3750/0.3800/polBen!36!white,0.3800/0.3850/polBen!36!white,0.3850/0.3900/polBen!33!white,0.3900/0.3950/polBen!33!white,0.3950/0.4000/polBen!33!white,0.4000/0.4050/polBen!33!white,0.4050/0.4100/polBen!33!white,0.4100/0.4150/polBen!33!white,0.4150/0.4200/polBen!31!white,0.4200/0.4250/polBen!31!white,0.4250/0.4300/polBen!31!white,0.4300/0.4350/polBen!28!white,0.4350/0.4400/polBen!25!white,0.4400/0.4450/polBen!25!white,0.4450/0.4500/polBen!25!white,0.4500/0.4550/polBen!25!white,0.4550/0.4600/polBen!22!white,0.4600/0.4650/polBen!13!white,0.4650/0.4700/polBen!13!white,0.4700/0.4750/polBen!13!white,0.4750/0.4800/polBen!13!white,0.4800/0.4850/polBen!13!white,0.4850/0.4900/polBen!13!white,0.4900/0.4950/polBen!0!white,0.4950/0.5000/polBen!0!white,0.5000/0.5050/polBen!0!white,0.5050/0.5100/polBen!0!white,0.5100/0.5150/polBen!0!white,0.5150/0.5200/polBen!0!white,0.5200/0.5250/polMal!0!white,0.5250/0.5300/polMal!0!white,0.5300/0.5350/polMal!0!white,0.5350/0.5400/polMal!12!white,0.5400/0.5450/polMal!12!white,0.5450/0.5500/polMal!12!white,0.5500/0.5550/polMal!16!white,0.5550/0.5600/polMal!20!white,0.5600/0.5650/polMal!23!white,0.5650/0.5700/polMal!26!white,0.5700/0.5750/polMal!31!white,0.5750/0.5800/polMal!31!white,0.5800/0.5850/polMal!35!white,0.5850/0.5900/polMal!37!white,0.5900/0.5950/polMal!37!white,0.5950/0.6000/polMal!38!white,0.6000/0.6050/polMal!40!white,0.6050/0.6100/polMal!40!white,0.6100/0.6150/polMal!40!white,0.6150/0.6200/polMal!43!white,0.6200/0.6250/polMal!45!white,0.6250/0.6300/polMal!46!white,0.6300/0.6350/polMal!48!white,0.6350/0.6400/polMal!48!white,0.6400/0.6450/polMal!48!white,0.6450/0.6500/polMal!49!white,0.6500/0.6550/polMal!50!white,0.6550/0.6600/polMal!50!white,0.6600/0.6650/polMal!50!white,0.6650/0.6700/polMal!52!white,0.6700/0.6750/polMal!52!white,0.6750/0.6800/polMal!52!white,0.6800/0.6850/polMal!53!white,0.6850/0.6900/polMal!53!white,0.6900/0.6950/polMal!53!white,0.6950/0.7000/polMal!54!white,0.7000/0.7050/polMal!54!white,0.7050/0.7100/polMal!55!white,0.7100/0.7150/polMal!55!white,0.7150/0.7200/polMal!58!white,0.7200/0.7250/polMal!58!white,0.7250/0.7300/polMal!61!white,0.7300/0.7350/polMal!62!white,0.7350/0.7400/polMal!62!white,0.7400/0.7450/polMal!62!white,0.7450/0.7500/polMal!64!white,0.7500/0.7550/polMal!65!white,0.7550/0.7600/polMal!65!white,0.7600/0.7650/polMal!66!white,0.7650/0.7700/polMal!66!white,0.7700/0.7750/polMal!66!white,0.7750/0.7800/polMal!66!white,0.7800/0.7850/polMal!67!white,0.7850/0.7900/polMal!68!white,0.7900/0.7950/polMal!68!white,0.7950/0.8000/polMal!70!white,0.8000/0.8050/polMal!71!white,0.8050/0.8100/polMal!71!white,0.8100/0.8150/polMal!72!white,0.8150/0.8200/polMal!72!white,0.8200/0.8250/polMal!72!white,0.8250/0.8300/polMal!73!white,0.8300/0.8350/polMal!73!white,0.8350/0.8400/polMal!73!white,0.8400/0.8450/polMal!73!white,0.8450/0.8500/polMal!73!white,0.8500/0.8550/polMal!73!white,0.8550/0.8600/polMal!75!white,0.8600/0.8650/polMal!75!white,0.8650/0.8700/polMal!75!white,0.8700/0.8750/polMal!75!white,0.8750/0.8800/polMal!76!white,0.8800/0.8850/polMal!76!white,0.8850/0.8900/polMal!77!white,0.8900/0.8950/polMal!77!white,0.8950/0.9000/polMal!77!white,0.9000/0.9050/polMal!79!white,0.9050/0.9100/polMal!79!white,0.9100/0.9150/polMal!80!white,0.9150/0.9200/polMal!81!white,0.9200/0.9250/polMal!81!white,0.9250/0.9300/polMal!82!white,0.9300/0.9350/polMal!82!white,0.9350/0.9400/polMal!83!white,0.9400/0.9450/polMal!84!white,0.9450/0.9500/polMal!84!white,0.9500/0.9550/polMal!84!white,0.9550/0.9600/polMal!84!white,0.9600/0.9650/polMal!85!white,0.9650/0.9700/polMal!86!white,0.9700/0.9750/polMal!87!white,0.9750/0.9800/polMal!87!white,0.9800/0.9850/polMal!87!white,0.9850/0.9900/polMal!90!white,0.9900/0.9950/polMal!91!white,0.9950/1.0000/polMal!100!white}
\def\polRAMmissing{0}
\def\polRAMarrows{0.2408/40.39/49.48/polBen,0.3892/25.88/38.18/polBen,0.7008/55.38/42.12/polMal,0.8825/71.77/54.46/polMal}
\def\polRAMhasarrows{1}
\def\polRAMben{39\,$\to$\,45\,\%}
\def\polRAMmal{59\,$\to$\,51\,\%}
\def\polRAMsplit{0.50833}
\def\polRAMn{466}
\def\polRAMev{307}
\def\polRAMC{600}
\def\polRAMstrip{0.0000/0.0017/polBen!100!white,0.0017/0.0033/polBen!99!white,0.0033/0.0050/polBen!97!white,0.0050/0.0067/polBen!96!white,0.0067/0.0083/polBen!96!white,0.0083/0.0100/polBen!95!white,0.0100/0.0117/polBen!95!white,0.0117/0.0133/polBen!95!white,0.0133/0.0150/polBen!94!white,0.0150/0.0167/polBen!94!white,0.0167/0.0183/polBen!94!white,0.0183/0.0200/polBen!94!white,0.0200/0.0217/polBen!93!white,0.0217/0.0233/polBen!93!white,0.0233/0.0250/polBen!93!white,0.0250/0.0267/polBen!92!white,0.0267/0.0283/polBen!92!white,0.0283/0.0300/polBen!92!white,0.0300/0.0317/polBen!91!white,0.0317/0.0333/polBen!91!white,0.0333/0.0350/polBen!91!white,0.0350/0.0367/polBen!91!white,0.0367/0.0383/polBen!91!white,0.0383/0.0400/polBen!91!white,0.0400/0.0417/polBen!90!white,0.0417/0.0433/polBen!89!white,0.0433/0.0450/polBen!89!white,0.0450/0.0467/polBen!89!white,0.0467/0.0483/polBen!89!white,0.0483/0.0500/polBen!88!white,0.0500/0.0517/polBen!88!white,0.0517/0.0533/polBen!87!white,0.0533/0.0550/polBen!87!white,0.0550/0.0567/polBen!87!white,0.0567/0.0583/polBen!87!white,0.0583/0.0600/polBen!86!white,0.0600/0.0617/polBen!86!white,0.0617/0.0633/polBen!86!white,0.0633/0.0650/polBen!86!white,0.0650/0.0667/polBen!86!white,0.0667/0.0683/polBen!85!white,0.0683/0.0700/polBen!85!white,0.0700/0.0717/polBen!85!white,0.0717/0.0733/polBen!85!white,0.0733/0.0750/polBen!84!white,0.0750/0.0767/polBen!83!white,0.0767/0.0783/polBen!83!white,0.0783/0.0800/polBen!83!white,0.0800/0.0817/polBen!83!white,0.0817/0.0833/polBen!83!white,0.0833/0.0850/polBen!83!white,0.0850/0.0867/polBen!83!white,0.0867/0.0883/polBen!83!white,0.0883/0.0900/polBen!83!white,0.0900/0.0917/polBen!83!white,0.0917/0.0933/polBen!82!white,0.0933/0.0950/polBen!82!white,0.0950/0.0967/polBen!82!white,0.0967/0.0983/polBen!82!white,0.0983/0.1000/polBen!82!white,0.1000/0.1017/polBen!82!white,0.1017/0.1033/polBen!82!white,0.1033/0.1050/polBen!82!white,0.1050/0.1067/polBen!82!white,0.1067/0.1083/polBen!82!white,0.1083/0.1100/polBen!82!white,0.1100/0.1117/polBen!82!white,0.1117/0.1133/polBen!81!white,0.1133/0.1150/polBen!81!white,0.1150/0.1167/polBen!81!white,0.1167/0.1183/polBen!81!white,0.1183/0.1200/polBen!81!white,0.1200/0.1217/polBen!81!white,0.1217/0.1233/polBen!81!white,0.1233/0.1250/polBen!81!white,0.1250/0.1267/polBen!80!white,0.1267/0.1283/polBen!80!white,0.1283/0.1300/polBen!80!white,0.1300/0.1317/polBen!80!white,0.1317/0.1333/polBen!80!white,0.1333/0.1350/polBen!80!white,0.1350/0.1367/polBen!80!white,0.1367/0.1383/polBen!79!white,0.1383/0.1400/polBen!79!white,0.1400/0.1417/polBen!79!white,0.1417/0.1433/polBen!79!white,0.1433/0.1450/polBen!79!white,0.1450/0.1467/polBen!79!white,0.1467/0.1483/polBen!78!white,0.1483/0.1500/polBen!78!white,0.1500/0.1517/polBen!78!white,0.1517/0.1533/polBen!78!white,0.1533/0.1550/polBen!78!white,0.1550/0.1567/polBen!78!white,0.1567/0.1583/polBen!78!white,0.1583/0.1600/polBen!78!white,0.1600/0.1617/polBen!78!white,0.1617/0.1633/polBen!78!white,0.1633/0.1650/polBen!78!white,0.1650/0.1667/polBen!77!white,0.1667/0.1683/polBen!77!white,0.1683/0.1700/polBen!77!white,0.1700/0.1717/polBen!77!white,0.1717/0.1733/polBen!77!white,0.1733/0.1750/polBen!77!white,0.1750/0.1767/polBen!77!white,0.1767/0.1783/polBen!77!white,0.1783/0.1800/polBen!77!white,0.1800/0.1817/polBen!77!white,0.1817/0.1833/polBen!76!white,0.1833/0.1850/polBen!76!white,0.1850/0.1867/polBen!76!white,0.1867/0.1883/polBen!76!white,0.1883/0.1900/polBen!75!white,0.1900/0.1917/polBen!75!white,0.1917/0.1933/polBen!75!white,0.1933/0.1950/polBen!75!white,0.1950/0.1967/polBen!75!white,0.1967/0.1983/polBen!75!white,0.1983/0.2000/polBen!75!white,0.2000/0.2017/polBen!75!white,0.2017/0.2033/polBen!74!white,0.2033/0.2050/polBen!74!white,0.2050/0.2067/polBen!74!white,0.2067/0.2083/polBen!74!white,0.2083/0.2100/polBen!74!white,0.2100/0.2117/polBen!74!white,0.2117/0.2133/polBen!73!white,0.2133/0.2150/polBen!73!white,0.2150/0.2167/polBen!73!white,0.2167/0.2183/polBen!73!white,0.2183/0.2200/polBen!73!white,0.2200/0.2217/polBen!72!white,0.2217/0.2233/polBen!72!white,0.2233/0.2250/polBen!72!white,0.2250/0.2267/polBen!72!white,0.2267/0.2283/polBen!72!white,0.2283/0.2300/polBen!72!white,0.2300/0.2317/polBen!72!white,0.2317/0.2333/polBen!72!white,0.2333/0.2350/polBen!71!white,0.2350/0.2367/polBen!71!white,0.2367/0.2383/polBen!71!white,0.2383/0.2400/polBen!71!white,0.2400/0.2417/polBen!71!white,0.2417/0.2433/polBen!71!white,0.2433/0.2450/polBen!70!white,0.2450/0.2467/polBen!70!white,0.2467/0.2483/polBen!70!white,0.2483/0.2500/polBen!70!white,0.2500/0.2517/polBen!70!white,0.2517/0.2533/polBen!70!white,0.2533/0.2550/polBen!70!white,0.2550/0.2567/polBen!69!white,0.2567/0.2583/polBen!69!white,0.2583/0.2600/polBen!69!white,0.2600/0.2617/polBen!69!white,0.2617/0.2633/polBen!68!white,0.2633/0.2650/polBen!68!white,0.2650/0.2667/polBen!68!white,0.2667/0.2683/polBen!68!white,0.2683/0.2700/polBen!68!white,0.2700/0.2717/polBen!68!white,0.2717/0.2733/polBen!68!white,0.2733/0.2750/polBen!68!white,0.2750/0.2767/polBen!68!white,0.2767/0.2783/polBen!68!white,0.2783/0.2800/polBen!68!white,0.2800/0.2817/polBen!68!white,0.2817/0.2833/polBen!67!white,0.2833/0.2850/polBen!67!white,0.2850/0.2867/polBen!67!white,0.2867/0.2883/polBen!67!white,0.2883/0.2900/polBen!67!white,0.2900/0.2917/polBen!67!white,0.2917/0.2933/polBen!67!white,0.2933/0.2950/polBen!66!white,0.2950/0.2967/polBen!66!white,0.2967/0.2983/polBen!66!white,0.2983/0.3000/polBen!66!white,0.3000/0.3017/polBen!65!white,0.3017/0.3033/polBen!65!white,0.3033/0.3050/polBen!65!white,0.3050/0.3067/polBen!65!white,0.3067/0.3083/polBen!65!white,0.3083/0.3100/polBen!65!white,0.3100/0.3117/polBen!65!white,0.3117/0.3133/polBen!64!white,0.3133/0.3150/polBen!64!white,0.3150/0.3167/polBen!64!white,0.3167/0.3183/polBen!64!white,0.3183/0.3200/polBen!64!white,0.3200/0.3217/polBen!64!white,0.3217/0.3233/polBen!63!white,0.3233/0.3250/polBen!63!white,0.3250/0.3267/polBen!63!white,0.3267/0.3283/polBen!63!white,0.3283/0.3300/polBen!63!white,0.3300/0.3317/polBen!62!white,0.3317/0.3333/polBen!62!white,0.3333/0.3350/polBen!62!white,0.3350/0.3367/polBen!62!white,0.3367/0.3383/polBen!62!white,0.3383/0.3400/polBen!62!white,0.3400/0.3417/polBen!62!white,0.3417/0.3433/polBen!61!white,0.3433/0.3450/polBen!61!white,0.3450/0.3467/polBen!61!white,0.3467/0.3483/polBen!61!white,0.3483/0.3500/polBen!61!white,0.3500/0.3517/polBen!61!white,0.3517/0.3533/polBen!61!white,0.3533/0.3550/polBen!61!white,0.3550/0.3567/polBen!61!white,0.3567/0.3583/polBen!60!white,0.3583/0.3600/polBen!60!white,0.3600/0.3617/polBen!60!white,0.3617/0.3633/polBen!60!white,0.3633/0.3650/polBen!59!white,0.3650/0.3667/polBen!59!white,0.3667/0.3683/polBen!59!white,0.3683/0.3700/polBen!59!white,0.3700/0.3717/polBen!59!white,0.3717/0.3733/polBen!59!white,0.3733/0.3750/polBen!58!white,0.3750/0.3767/polBen!58!white,0.3767/0.3783/polBen!58!white,0.3783/0.3800/polBen!58!white,0.3800/0.3817/polBen!58!white,0.3817/0.3833/polBen!57!white,0.3833/0.3850/polBen!57!white,0.3850/0.3867/polBen!57!white,0.3867/0.3883/polBen!57!white,0.3883/0.3900/polBen!57!white,0.3900/0.3917/polBen!56!white,0.3917/0.3933/polBen!56!white,0.3933/0.3950/polBen!56!white,0.3950/0.3967/polBen!56!white,0.3967/0.3983/polBen!56!white,0.3983/0.4000/polBen!56!white,0.4000/0.4017/polBen!55!white,0.4017/0.4033/polBen!55!white,0.4033/0.4050/polBen!55!white,0.4050/0.4067/polBen!55!white,0.4067/0.4083/polBen!55!white,0.4083/0.4100/polBen!54!white,0.4100/0.4117/polBen!54!white,0.4117/0.4133/polBen!54!white,0.4133/0.4150/polBen!54!white,0.4150/0.4167/polBen!54!white,0.4167/0.4183/polBen!53!white,0.4183/0.4200/polBen!53!white,0.4200/0.4217/polBen!53!white,0.4217/0.4233/polBen!53!white,0.4233/0.4250/polBen!53!white,0.4250/0.4267/polBen!53!white,0.4267/0.4283/polBen!53!white,0.4283/0.4300/polBen!52!white,0.4300/0.4317/polBen!52!white,0.4317/0.4333/polBen!52!white,0.4333/0.4350/polBen!52!white,0.4350/0.4367/polBen!51!white,0.4367/0.4383/polBen!51!white,0.4383/0.4400/polBen!51!white,0.4400/0.4417/polBen!51!white,0.4417/0.4433/polBen!50!white,0.4433/0.4450/polBen!50!white,0.4450/0.4467/polBen!50!white,0.4467/0.4483/polBen!49!white,0.4483/0.4500/polBen!49!white,0.4500/0.4517/polBen!49!white,0.4517/0.4533/polBen!49!white,0.4533/0.4550/polBen!48!white,0.4550/0.4567/polBen!48!white,0.4567/0.4583/polBen!47!white,0.4583/0.4600/polBen!47!white,0.4600/0.4617/polBen!47!white,0.4617/0.4633/polBen!46!white,0.4633/0.4650/polBen!46!white,0.4650/0.4667/polBen!46!white,0.4667/0.4683/polBen!44!white,0.4683/0.4700/polBen!44!white,0.4700/0.4717/polBen!44!white,0.4717/0.4733/polBen!43!white,0.4733/0.4750/polBen!42!white,0.4750/0.4767/polBen!42!white,0.4767/0.4783/polBen!41!white,0.4783/0.4800/polBen!41!white,0.4800/0.4817/polBen!41!white,0.4817/0.4833/polBen!41!white,0.4833/0.4850/polBen!40!white,0.4850/0.4867/polBen!39!white,0.4867/0.4883/polBen!37!white,0.4883/0.4900/polBen!37!white,0.4900/0.4917/polBen!35!white,0.4917/0.4933/polBen!35!white,0.4933/0.4950/polBen!35!white,0.4950/0.4967/polBen!35!white,0.4967/0.4983/polBen!33!white,0.4983/0.5000/polBen!33!white,0.5000/0.5017/polBen!31!white,0.5017/0.5033/polBen!30!white,0.5033/0.5050/polBen!27!white,0.5050/0.5067/polBen!26!white,0.5067/0.5083/polBen!25!white,0.5083/0.5100/polMal!34!white,0.5100/0.5117/polMal!41!white,0.5117/0.5133/polMal!44!white,0.5133/0.5150/polMal!44!white,0.5150/0.5167/polMal!45!white,0.5167/0.5183/polMal!49!white,0.5183/0.5200/polMal!51!white,0.5200/0.5217/polMal!51!white,0.5217/0.5233/polMal!52!white,0.5233/0.5250/polMal!52!white,0.5250/0.5267/polMal!53!white,0.5267/0.5283/polMal!53!white,0.5283/0.5300/polMal!54!white,0.5300/0.5317/polMal!55!white,0.5317/0.5333/polMal!55!white,0.5333/0.5350/polMal!56!white,0.5350/0.5367/polMal!57!white,0.5367/0.5383/polMal!57!white,0.5383/0.5400/polMal!58!white,0.5400/0.5417/polMal!59!white,0.5417/0.5433/polMal!59!white,0.5433/0.5450/polMal!59!white,0.5450/0.5467/polMal!60!white,0.5467/0.5483/polMal!60!white,0.5483/0.5500/polMal!60!white,0.5500/0.5517/polMal!60!white,0.5517/0.5533/polMal!61!white,0.5533/0.5550/polMal!62!white,0.5550/0.5567/polMal!62!white,0.5567/0.5583/polMal!62!white,0.5583/0.5600/polMal!63!white,0.5600/0.5617/polMal!63!white,0.5617/0.5633/polMal!63!white,0.5633/0.5650/polMal!63!white,0.5650/0.5667/polMal!63!white,0.5667/0.5683/polMal!64!white,0.5683/0.5700/polMal!64!white,0.5700/0.5717/polMal!64!white,0.5717/0.5733/polMal!64!white,0.5733/0.5750/polMal!64!white,0.5750/0.5767/polMal!64!white,0.5767/0.5783/polMal!65!white,0.5783/0.5800/polMal!65!white,0.5800/0.5817/polMal!65!white,0.5817/0.5833/polMal!65!white,0.5833/0.5850/polMal!65!white,0.5850/0.5867/polMal!66!white,0.5867/0.5883/polMal!66!white,0.5883/0.5900/polMal!66!white,0.5900/0.5917/polMal!66!white,0.5917/0.5933/polMal!67!white,0.5933/0.5950/polMal!67!white,0.5950/0.5967/polMal!67!white,0.5967/0.5983/polMal!67!white,0.5983/0.6000/polMal!67!white,0.6000/0.6017/polMal!67!white,0.6017/0.6033/polMal!68!white,0.6033/0.6050/polMal!68!white,0.6050/0.6067/polMal!68!white,0.6067/0.6083/polMal!69!white,0.6083/0.6100/polMal!69!white,0.6100/0.6117/polMal!69!white,0.6117/0.6133/polMal!70!white,0.6133/0.6150/polMal!70!white,0.6150/0.6167/polMal!70!white,0.6167/0.6183/polMal!70!white,0.6183/0.6200/polMal!70!white,0.6200/0.6217/polMal!71!white,0.6217/0.6233/polMal!71!white,0.6233/0.6250/polMal!71!white,0.6250/0.6267/polMal!71!white,0.6267/0.6283/polMal!71!white,0.6283/0.6300/polMal!72!white,0.6300/0.6317/polMal!72!white,0.6317/0.6333/polMal!72!white,0.6333/0.6350/polMal!72!white,0.6350/0.6367/polMal!72!white,0.6367/0.6383/polMal!72!white,0.6383/0.6400/polMal!72!white,0.6400/0.6417/polMal!72!white,0.6417/0.6433/polMal!72!white,0.6433/0.6450/polMal!72!white,0.6450/0.6467/polMal!73!white,0.6467/0.6483/polMal!73!white,0.6483/0.6500/polMal!73!white,0.6500/0.6517/polMal!73!white,0.6517/0.6533/polMal!73!white,0.6533/0.6550/polMal!73!white,0.6550/0.6567/polMal!73!white,0.6567/0.6583/polMal!74!white,0.6583/0.6600/polMal!74!white,0.6600/0.6617/polMal!74!white,0.6617/0.6633/polMal!74!white,0.6633/0.6650/polMal!74!white,0.6650/0.6667/polMal!74!white,0.6667/0.6683/polMal!74!white,0.6683/0.6700/polMal!74!white,0.6700/0.6717/polMal!75!white,0.6717/0.6733/polMal!75!white,0.6733/0.6750/polMal!75!white,0.6750/0.6767/polMal!75!white,0.6767/0.6783/polMal!75!white,0.6783/0.6800/polMal!75!white,0.6800/0.6817/polMal!75!white,0.6817/0.6833/polMal!76!white,0.6833/0.6850/polMal!76!white,0.6850/0.6867/polMal!76!white,0.6867/0.6883/polMal!76!white,0.6883/0.6900/polMal!76!white,0.6900/0.6917/polMal!76!white,0.6917/0.6933/polMal!76!white,0.6933/0.6950/polMal!76!white,0.6950/0.6967/polMal!76!white,0.6967/0.6983/polMal!77!white,0.6983/0.7000/polMal!77!white,0.7000/0.7017/polMal!77!white,0.7017/0.7033/polMal!77!white,0.7033/0.7050/polMal!77!white,0.7050/0.7067/polMal!77!white,0.7067/0.7083/polMal!78!white,0.7083/0.7100/polMal!78!white,0.7100/0.7117/polMal!78!white,0.7117/0.7133/polMal!78!white,0.7133/0.7150/polMal!78!white,0.7150/0.7167/polMal!78!white,0.7167/0.7183/polMal!78!white,0.7183/0.7200/polMal!78!white,0.7200/0.7217/polMal!78!white,0.7217/0.7233/polMal!78!white,0.7233/0.7250/polMal!79!white,0.7250/0.7267/polMal!79!white,0.7267/0.7283/polMal!79!white,0.7283/0.7300/polMal!79!white,0.7300/0.7317/polMal!79!white,0.7317/0.7333/polMal!79!white,0.7333/0.7350/polMal!79!white,0.7350/0.7367/polMal!80!white,0.7367/0.7383/polMal!80!white,0.7383/0.7400/polMal!80!white,0.7400/0.7417/polMal!80!white,0.7417/0.7433/polMal!80!white,0.7433/0.7450/polMal!80!white,0.7450/0.7467/polMal!80!white,0.7467/0.7483/polMal!80!white,0.7483/0.7500/polMal!80!white,0.7500/0.7517/polMal!81!white,0.7517/0.7533/polMal!81!white,0.7533/0.7550/polMal!81!white,0.7550/0.7567/polMal!81!white,0.7567/0.7583/polMal!81!white,0.7583/0.7600/polMal!81!white,0.7600/0.7617/polMal!81!white,0.7617/0.7633/polMal!81!white,0.7633/0.7650/polMal!81!white,0.7650/0.7667/polMal!81!white,0.7667/0.7683/polMal!81!white,0.7683/0.7700/polMal!82!white,0.7700/0.7717/polMal!82!white,0.7717/0.7733/polMal!82!white,0.7733/0.7750/polMal!82!white,0.7750/0.7767/polMal!82!white,0.7767/0.7783/polMal!82!white,0.7783/0.7800/polMal!82!white,0.7800/0.7817/polMal!82!white,0.7817/0.7833/polMal!82!white,0.7833/0.7850/polMal!82!white,0.7850/0.7867/polMal!82!white,0.7867/0.7883/polMal!82!white,0.7883/0.7900/polMal!82!white,0.7900/0.7917/polMal!82!white,0.7917/0.7933/polMal!82!white,0.7933/0.7950/polMal!83!white,0.7950/0.7967/polMal!83!white,0.7967/0.7983/polMal!83!white,0.7983/0.8000/polMal!83!white,0.8000/0.8017/polMal!83!white,0.8017/0.8033/polMal!83!white,0.8033/0.8050/polMal!83!white,0.8050/0.8067/polMal!83!white,0.8067/0.8083/polMal!83!white,0.8083/0.8100/polMal!83!white,0.8100/0.8117/polMal!83!white,0.8117/0.8133/polMal!83!white,0.8133/0.8150/polMal!83!white,0.8150/0.8167/polMal!83!white,0.8167/0.8183/polMal!83!white,0.8183/0.8200/polMal!83!white,0.8200/0.8217/polMal!84!white,0.8217/0.8233/polMal!84!white,0.8233/0.8250/polMal!84!white,0.8250/0.8267/polMal!84!white,0.8267/0.8283/polMal!84!white,0.8283/0.8300/polMal!84!white,0.8300/0.8317/polMal!84!white,0.8317/0.8333/polMal!84!white,0.8333/0.8350/polMal!84!white,0.8350/0.8367/polMal!84!white,0.8367/0.8383/polMal!84!white,0.8383/0.8400/polMal!84!white,0.8400/0.8417/polMal!84!white,0.8417/0.8433/polMal!85!white,0.8433/0.8450/polMal!85!white,0.8450/0.8467/polMal!85!white,0.8467/0.8483/polMal!85!white,0.8483/0.8500/polMal!85!white,0.8500/0.8517/polMal!86!white,0.8517/0.8533/polMal!86!white,0.8533/0.8550/polMal!86!white,0.8550/0.8567/polMal!86!white,0.8567/0.8583/polMal!86!white,0.8583/0.8600/polMal!86!white,0.8600/0.8617/polMal!86!white,0.8617/0.8633/polMal!86!white,0.8633/0.8650/polMal!86!white,0.8650/0.8667/polMal!87!white,0.8667/0.8683/polMal!87!white,0.8683/0.8700/polMal!87!white,0.8700/0.8717/polMal!87!white,0.8717/0.8733/polMal!87!white,0.8733/0.8750/polMal!87!white,0.8750/0.8767/polMal!87!white,0.8767/0.8783/polMal!87!white,0.8783/0.8800/polMal!87!white,0.8800/0.8817/polMal!87!white,0.8817/0.8833/polMal!88!white,0.8833/0.8850/polMal!88!white,0.8850/0.8867/polMal!88!white,0.8867/0.8883/polMal!88!white,0.8883/0.8900/polMal!88!white,0.8900/0.8917/polMal!88!white,0.8917/0.8933/polMal!88!white,0.8933/0.8950/polMal!88!white,0.8950/0.8967/polMal!88!white,0.8967/0.8983/polMal!88!white,0.8983/0.9000/polMal!89!white,0.9000/0.9017/polMal!89!white,0.9017/0.9033/polMal!89!white,0.9033/0.9050/polMal!89!white,0.9050/0.9067/polMal!89!white,0.9067/0.9083/polMal!89!white,0.9083/0.9100/polMal!89!white,0.9100/0.9117/polMal!89!white,0.9117/0.9133/polMal!89!white,0.9133/0.9150/polMal!89!white,0.9150/0.9167/polMal!90!white,0.9167/0.9183/polMal!90!white,0.9183/0.9200/polMal!90!white,0.9200/0.9217/polMal!90!white,0.9217/0.9233/polMal!90!white,0.9233/0.9250/polMal!90!white,0.9250/0.9267/polMal!91!white,0.9267/0.9283/polMal!91!white,0.9283/0.9300/polMal!91!white,0.9300/0.9317/polMal!91!white,0.9317/0.9333/polMal!91!white,0.9333/0.9350/polMal!91!white,0.9350/0.9367/polMal!91!white,0.9367/0.9383/polMal!92!white,0.9383/0.9400/polMal!92!white,0.9400/0.9417/polMal!92!white,0.9417/0.9433/polMal!92!white,0.9433/0.9450/polMal!92!white,0.9450/0.9467/polMal!92!white,0.9467/0.9483/polMal!92!white,0.9483/0.9500/polMal!92!white,0.9500/0.9517/polMal!92!white,0.9517/0.9533/polMal!92!white,0.9533/0.9550/polMal!92!white,0.9550/0.9567/polMal!92!white,0.9567/0.9583/polMal!93!white,0.9583/0.9600/polMal!93!white,0.9600/0.9617/polMal!93!white,0.9617/0.9633/polMal!93!white,0.9633/0.9650/polMal!93!white,0.9650/0.9667/polMal!94!white,0.9667/0.9683/polMal!94!white,0.9683/0.9700/polMal!94!white,0.9700/0.9717/polMal!94!white,0.9717/0.9733/polMal!94!white,0.9733/0.9750/polMal!94!white,0.9750/0.9767/polMal!94!white,0.9767/0.9783/polMal!94!white,0.9783/0.9800/polMal!94!white,0.9800/0.9817/polMal!94!white,0.9817/0.9833/polMal!95!white,0.9833/0.9850/polMal!95!white,0.9850/0.9867/polMal!95!white,0.9867/0.9883/polMal!95!white,0.9883/0.9900/polMal!95!white,0.9900/0.9917/polMal!97!white,0.9917/0.9933/polMal!97!white,0.9933/0.9950/polMal!97!white,0.9950/0.9967/polMal!98!white,0.9967/0.9983/polMal!100!white,0.9983/1.0000/polMal!100!white}
\def\polHCCmissing{0}
\def\polHCCarrows{0.8760/11.58/6.30/polMal}
\def\polHCChasarrows{1}
\def\polHCCben{8\,$\to$\,9\,\%}
\def\polHCCmal{8\,$\to$\,7\,\%}
\def\polHCCsplit{0.49414}
\def\polHCCn{221}
\def\polHCCev{221}
\def\polHCCC{512}
\def\polHCCstrip{0.0000/0.0020/polBen!100!white,0.0020/0.0039/polBen!85!white,0.0039/0.0059/polBen!72!white,0.0059/0.0078/polBen!71!white,0.0078/0.0098/polBen!65!white,0.0098/0.0117/polBen!61!white,0.0117/0.0137/polBen!60!white,0.0137/0.0156/polBen!59!white,0.0156/0.0176/polBen!58!white,0.0176/0.0195/polBen!57!white,0.0195/0.0215/polBen!57!white,0.0215/0.0234/polBen!53!white,0.0234/0.0254/polBen!52!white,0.0254/0.0273/polBen!50!white,0.0273/0.0293/polBen!49!white,0.0293/0.0312/polBen!48!white,0.0312/0.0332/polBen!48!white,0.0332/0.0352/polBen!47!white,0.0352/0.0371/polBen!47!white,0.0371/0.0391/polBen!47!white,0.0391/0.0410/polBen!46!white,0.0410/0.0430/polBen!46!white,0.0430/0.0449/polBen!46!white,0.0449/0.0469/polBen!45!white,0.0469/0.0488/polBen!45!white,0.0488/0.0508/polBen!45!white,0.0508/0.0527/polBen!44!white,0.0527/0.0547/polBen!44!white,0.0547/0.0566/polBen!44!white,0.0566/0.0586/polBen!43!white,0.0586/0.0605/polBen!42!white,0.0605/0.0625/polBen!42!white,0.0625/0.0645/polBen!42!white,0.0645/0.0664/polBen!42!white,0.0664/0.0684/polBen!41!white,0.0684/0.0703/polBen!41!white,0.0703/0.0723/polBen!41!white,0.0723/0.0742/polBen!41!white,0.0742/0.0762/polBen!41!white,0.0762/0.0781/polBen!41!white,0.0781/0.0801/polBen!41!white,0.0801/0.0820/polBen!41!white,0.0820/0.0840/polBen!41!white,0.0840/0.0859/polBen!40!white,0.0859/0.0879/polBen!40!white,0.0879/0.0898/polBen!39!white,0.0898/0.0918/polBen!39!white,0.0918/0.0938/polBen!38!white,0.0938/0.0957/polBen!38!white,0.0957/0.0977/polBen!38!white,0.0977/0.0996/polBen!38!white,0.0996/0.1016/polBen!38!white,0.1016/0.1035/polBen!36!white,0.1035/0.1055/polBen!36!white,0.1055/0.1074/polBen!36!white,0.1074/0.1094/polBen!36!white,0.1094/0.1113/polBen!35!white,0.1113/0.1133/polBen!35!white,0.1133/0.1152/polBen!35!white,0.1152/0.1172/polBen!35!white,0.1172/0.1191/polBen!34!white,0.1191/0.1211/polBen!34!white,0.1211/0.1230/polBen!34!white,0.1230/0.1250/polBen!34!white,0.1250/0.1270/polBen!33!white,0.1270/0.1289/polBen!33!white,0.1289/0.1309/polBen!33!white,0.1309/0.1328/polBen!33!white,0.1328/0.1348/polBen!33!white,0.1348/0.1367/polBen!33!white,0.1367/0.1387/polBen!33!white,0.1387/0.1406/polBen!33!white,0.1406/0.1426/polBen!32!white,0.1426/0.1445/polBen!32!white,0.1445/0.1465/polBen!32!white,0.1465/0.1484/polBen!32!white,0.1484/0.1504/polBen!32!white,0.1504/0.1523/polBen!31!white,0.1523/0.1543/polBen!31!white,0.1543/0.1562/polBen!31!white,0.1562/0.1582/polBen!31!white,0.1582/0.1602/polBen!31!white,0.1602/0.1621/polBen!31!white,0.1621/0.1641/polBen!31!white,0.1641/0.1660/polBen!30!white,0.1660/0.1680/polBen!30!white,0.1680/0.1699/polBen!30!white,0.1699/0.1719/polBen!30!white,0.1719/0.1738/polBen!30!white,0.1738/0.1758/polBen!30!white,0.1758/0.1777/polBen!30!white,0.1777/0.1797/polBen!30!white,0.1797/0.1816/polBen!30!white,0.1816/0.1836/polBen!29!white,0.1836/0.1855/polBen!29!white,0.1855/0.1875/polBen!29!white,0.1875/0.1895/polBen!29!white,0.1895/0.1914/polBen!29!white,0.1914/0.1934/polBen!28!white,0.1934/0.1953/polBen!28!white,0.1953/0.1973/polBen!28!white,0.1973/0.1992/polBen!28!white,0.1992/0.2012/polBen!27!white,0.2012/0.2031/polBen!27!white,0.2031/0.2051/polBen!27!white,0.2051/0.2070/polBen!27!white,0.2070/0.2090/polBen!27!white,0.2090/0.2109/polBen!27!white,0.2109/0.2129/polBen!27!white,0.2129/0.2148/polBen!27!white,0.2148/0.2168/polBen!27!white,0.2168/0.2188/polBen!27!white,0.2188/0.2207/polBen!27!white,0.2207/0.2227/polBen!26!white,0.2227/0.2246/polBen!26!white,0.2246/0.2266/polBen!26!white,0.2266/0.2285/polBen!26!white,0.2285/0.2305/polBen!26!white,0.2305/0.2324/polBen!26!white,0.2324/0.2344/polBen!26!white,0.2344/0.2363/polBen!26!white,0.2363/0.2383/polBen!26!white,0.2383/0.2402/polBen!26!white,0.2402/0.2422/polBen!26!white,0.2422/0.2441/polBen!25!white,0.2441/0.2461/polBen!25!white,0.2461/0.2480/polBen!25!white,0.2480/0.2500/polBen!25!white,0.2500/0.2520/polBen!25!white,0.2520/0.2539/polBen!25!white,0.2539/0.2559/polBen!25!white,0.2559/0.2578/polBen!25!white,0.2578/0.2598/polBen!25!white,0.2598/0.2617/polBen!25!white,0.2617/0.2637/polBen!24!white,0.2637/0.2656/polBen!24!white,0.2656/0.2676/polBen!24!white,0.2676/0.2695/polBen!24!white,0.2695/0.2715/polBen!23!white,0.2715/0.2734/polBen!23!white,0.2734/0.2754/polBen!23!white,0.2754/0.2773/polBen!23!white,0.2773/0.2793/polBen!23!white,0.2793/0.2812/polBen!23!white,0.2812/0.2832/polBen!23!white,0.2832/0.2852/polBen!23!white,0.2852/0.2871/polBen!22!white,0.2871/0.2891/polBen!22!white,0.2891/0.2910/polBen!22!white,0.2910/0.2930/polBen!22!white,0.2930/0.2949/polBen!21!white,0.2949/0.2969/polBen!21!white,0.2969/0.2988/polBen!21!white,0.2988/0.3008/polBen!21!white,0.3008/0.3027/polBen!20!white,0.3027/0.3047/polBen!20!white,0.3047/0.3066/polBen!20!white,0.3066/0.3086/polBen!20!white,0.3086/0.3105/polBen!20!white,0.3105/0.3125/polBen!18!white,0.3125/0.3145/polBen!18!white,0.3145/0.3164/polBen!18!white,0.3164/0.3184/polBen!18!white,0.3184/0.3203/polBen!18!white,0.3203/0.3223/polBen!17!white,0.3223/0.3242/polBen!17!white,0.3242/0.3262/polBen!17!white,0.3262/0.3281/polBen!17!white,0.3281/0.3301/polBen!17!white,0.3301/0.3320/polBen!16!white,0.3320/0.3340/polBen!16!white,0.3340/0.3359/polBen!16!white,0.3359/0.3379/polBen!16!white,0.3379/0.3398/polBen!16!white,0.3398/0.3418/polBen!16!white,0.3418/0.3438/polBen!16!white,0.3438/0.3457/polBen!14!white,0.3457/0.3477/polBen!14!white,0.3477/0.3496/polBen!14!white,0.3496/0.3516/polBen!14!white,0.3516/0.3535/polBen!14!white,0.3535/0.3555/polBen!14!white,0.3555/0.3574/polBen!14!white,0.3574/0.3594/polBen!12!white,0.3594/0.3613/polBen!12!white,0.3613/0.3633/polBen!12!white,0.3633/0.3652/polBen!12!white,0.3652/0.3672/polBen!12!white,0.3672/0.3691/polBen!12!white,0.3691/0.3711/polBen!12!white,0.3711/0.3730/polBen!12!white,0.3730/0.3750/polBen!12!white,0.3750/0.3770/polBen!10!white,0.3770/0.3789/polBen!10!white,0.3789/0.3809/polBen!10!white,0.3809/0.3828/polBen!10!white,0.3828/0.3848/polBen!10!white,0.3848/0.3867/polBen!10!white,0.3867/0.3887/polBen!10!white,0.3887/0.3906/polBen!10!white,0.3906/0.3926/polBen!10!white,0.3926/0.3945/polBen!7!white,0.3945/0.3965/polBen!7!white,0.3965/0.3984/polBen!7!white,0.3984/0.4004/polBen!7!white,0.4004/0.4023/polBen!7!white,0.4023/0.4043/polBen!7!white,0.4043/0.4062/polBen!7!white,0.4062/0.4082/polBen!7!white,0.4082/0.4102/polBen!7!white,0.4102/0.4121/polBen!0!white,0.4121/0.4141/polBen!0!white,0.4141/0.4160/polBen!0!white,0.4160/0.4180/polBen!0!white,0.4180/0.4199/polBen!0!white,0.4199/0.4219/polBen!0!white,0.4219/0.4238/polBen!0!white,0.4238/0.4258/polBen!0!white,0.4258/0.4277/polBen!0!white,0.4277/0.4297/polBen!0!white,0.4297/0.4316/polBen!0!white,0.4316/0.4336/polBen!0!white,0.4336/0.4355/polBen!0!white,0.4355/0.4375/polBen!0!white,0.4375/0.4395/polBen!0!white,0.4395/0.4414/polBen!0!white,0.4414/0.4434/polBen!0!white,0.4434/0.4453/polBen!0!white,0.4453/0.4473/polBen!0!white,0.4473/0.4492/polBen!0!white,0.4492/0.4512/polBen!0!white,0.4512/0.4531/polBen!0!white,0.4531/0.4551/polBen!0!white,0.4551/0.4570/polBen!0!white,0.4570/0.4590/polBen!0!white,0.4590/0.4609/polBen!0!white,0.4609/0.4629/polBen!0!white,0.4629/0.4648/polBen!0!white,0.4648/0.4668/polBen!0!white,0.4668/0.4688/polBen!0!white,0.4688/0.4707/polBen!0!white,0.4707/0.4727/polBen!0!white,0.4727/0.4746/polBen!0!white,0.4746/0.4766/polBen!0!white,0.4766/0.4785/polBen!0!white,0.4785/0.4805/polBen!0!white,0.4805/0.4824/polBen!0!white,0.4824/0.4844/polBen!0!white,0.4844/0.4863/polBen!0!white,0.4863/0.4883/polBen!0!white,0.4883/0.4902/polBen!0!white,0.4902/0.4922/polBen!0!white,0.4922/0.4941/polBen!0!white,0.4941/0.4961/polMal!0!white,0.4961/0.4980/polMal!0!white,0.4980/0.5000/polMal!0!white,0.5000/0.5020/polMal!0!white,0.5020/0.5039/polMal!0!white,0.5039/0.5059/polMal!0!white,0.5059/0.5078/polMal!0!white,0.5078/0.5098/polMal!0!white,0.5098/0.5117/polMal!0!white,0.5117/0.5137/polMal!0!white,0.5137/0.5156/polMal!0!white,0.5156/0.5176/polMal!0!white,0.5176/0.5195/polMal!0!white,0.5195/0.5215/polMal!0!white,0.5215/0.5234/polMal!0!white,0.5234/0.5254/polMal!0!white,0.5254/0.5273/polMal!0!white,0.5273/0.5293/polMal!0!white,0.5293/0.5312/polMal!0!white,0.5312/0.5332/polMal!0!white,0.5332/0.5352/polMal!0!white,0.5352/0.5371/polMal!0!white,0.5371/0.5391/polMal!0!white,0.5391/0.5410/polMal!0!white,0.5410/0.5430/polMal!0!white,0.5430/0.5449/polMal!0!white,0.5449/0.5469/polMal!0!white,0.5469/0.5488/polMal!0!white,0.5488/0.5508/polMal!0!white,0.5508/0.5527/polMal!0!white,0.5527/0.5547/polMal!0!white,0.5547/0.5566/polMal!0!white,0.5566/0.5586/polMal!0!white,0.5586/0.5605/polMal!0!white,0.5605/0.5625/polMal!0!white,0.5625/0.5645/polMal!0!white,0.5645/0.5664/polMal!0!white,0.5664/0.5684/polMal!0!white,0.5684/0.5703/polMal!0!white,0.5703/0.5723/polMal!0!white,0.5723/0.5742/polMal!0!white,0.5742/0.5762/polMal!0!white,0.5762/0.5781/polMal!0!white,0.5781/0.5801/polMal!0!white,0.5801/0.5820/polMal!0!white,0.5820/0.5840/polMal!0!white,0.5840/0.5859/polMal!0!white,0.5859/0.5879/polMal!0!white,0.5879/0.5898/polMal!0!white,0.5898/0.5918/polMal!0!white,0.5918/0.5938/polMal!0!white,0.5938/0.5957/polMal!0!white,0.5957/0.5977/polMal!0!white,0.5977/0.5996/polMal!0!white,0.5996/0.6016/polMal!0!white,0.6016/0.6035/polMal!0!white,0.6035/0.6055/polMal!0!white,0.6055/0.6074/polMal!0!white,0.6074/0.6094/polMal!0!white,0.6094/0.6113/polMal!0!white,0.6113/0.6133/polMal!0!white,0.6133/0.6152/polMal!0!white,0.6152/0.6172/polMal!0!white,0.6172/0.6191/polMal!0!white,0.6191/0.6211/polMal!0!white,0.6211/0.6230/polMal!0!white,0.6230/0.6250/polMal!0!white,0.6250/0.6270/polMal!7!white,0.6270/0.6289/polMal!7!white,0.6289/0.6309/polMal!7!white,0.6309/0.6328/polMal!7!white,0.6328/0.6348/polMal!7!white,0.6348/0.6367/polMal!7!white,0.6367/0.6387/polMal!7!white,0.6387/0.6406/polMal!7!white,0.6406/0.6426/polMal!7!white,0.6426/0.6445/polMal!10!white,0.6445/0.6465/polMal!10!white,0.6465/0.6484/polMal!10!white,0.6484/0.6504/polMal!10!white,0.6504/0.6523/polMal!10!white,0.6523/0.6543/polMal!10!white,0.6543/0.6562/polMal!10!white,0.6562/0.6582/polMal!10!white,0.6582/0.6602/polMal!10!white,0.6602/0.6621/polMal!10!white,0.6621/0.6641/polMal!12!white,0.6641/0.6660/polMal!12!white,0.6660/0.6680/polMal!12!white,0.6680/0.6699/polMal!12!white,0.6699/0.6719/polMal!12!white,0.6719/0.6738/polMal!12!white,0.6738/0.6758/polMal!12!white,0.6758/0.6777/polMal!12!white,0.6777/0.6797/polMal!12!white,0.6797/0.6816/polMal!12!white,0.6816/0.6836/polMal!12!white,0.6836/0.6855/polMal!12!white,0.6855/0.6875/polMal!13!white,0.6875/0.6895/polMal!13!white,0.6895/0.6914/polMal!13!white,0.6914/0.6934/polMal!13!white,0.6934/0.6953/polMal!13!white,0.6953/0.6973/polMal!15!white,0.6973/0.6992/polMal!15!white,0.6992/0.7012/polMal!15!white,0.7012/0.7031/polMal!15!white,0.7031/0.7051/polMal!16!white,0.7051/0.7070/polMal!16!white,0.7070/0.7090/polMal!16!white,0.7090/0.7109/polMal!16!white,0.7109/0.7129/polMal!16!white,0.7129/0.7148/polMal!16!white,0.7148/0.7168/polMal!16!white,0.7168/0.7188/polMal!18!white,0.7188/0.7207/polMal!18!white,0.7207/0.7227/polMal!18!white,0.7227/0.7246/polMal!18!white,0.7246/0.7266/polMal!18!white,0.7266/0.7285/polMal!19!white,0.7285/0.7305/polMal!20!white,0.7305/0.7324/polMal!20!white,0.7324/0.7344/polMal!20!white,0.7344/0.7363/polMal!20!white,0.7363/0.7383/polMal!20!white,0.7383/0.7402/polMal!21!white,0.7402/0.7422/polMal!21!white,0.7422/0.7441/polMal!21!white,0.7441/0.7461/polMal!21!white,0.7461/0.7480/polMal!21!white,0.7480/0.7500/polMal!21!white,0.7500/0.7520/polMal!21!white,0.7520/0.7539/polMal!21!white,0.7539/0.7559/polMal!21!white,0.7559/0.7578/polMal!22!white,0.7578/0.7598/polMal!22!white,0.7598/0.7617/polMal!22!white,0.7617/0.7637/polMal!22!white,0.7637/0.7656/polMal!22!white,0.7656/0.7676/polMal!23!white,0.7676/0.7695/polMal!23!white,0.7695/0.7715/polMal!23!white,0.7715/0.7734/polMal!24!white,0.7734/0.7754/polMal!24!white,0.7754/0.7773/polMal!24!white,0.7773/0.7793/polMal!24!white,0.7793/0.7812/polMal!24!white,0.7812/0.7832/polMal!25!white,0.7832/0.7852/polMal!25!white,0.7852/0.7871/polMal!25!white,0.7871/0.7891/polMal!25!white,0.7891/0.7910/polMal!25!white,0.7910/0.7930/polMal!26!white,0.7930/0.7949/polMal!26!white,0.7949/0.7969/polMal!26!white,0.7969/0.7988/polMal!27!white,0.7988/0.8008/polMal!27!white,0.8008/0.8027/polMal!27!white,0.8027/0.8047/polMal!28!white,0.8047/0.8066/polMal!28!white,0.8066/0.8086/polMal!28!white,0.8086/0.8105/polMal!28!white,0.8105/0.8125/polMal!28!white,0.8125/0.8145/polMal!28!white,0.8145/0.8164/polMal!28!white,0.8164/0.8184/polMal!29!white,0.8184/0.8203/polMal!29!white,0.8203/0.8223/polMal!29!white,0.8223/0.8242/polMal!29!white,0.8242/0.8262/polMal!29!white,0.8262/0.8281/polMal!29!white,0.8281/0.8301/polMal!29!white,0.8301/0.8320/polMal!29!white,0.8320/0.8340/polMal!29!white,0.8340/0.8359/polMal!29!white,0.8359/0.8379/polMal!30!white,0.8379/0.8398/polMal!31!white,0.8398/0.8418/polMal!31!white,0.8418/0.8438/polMal!31!white,0.8438/0.8457/polMal!31!white,0.8457/0.8477/polMal!32!white,0.8477/0.8496/polMal!32!white,0.8496/0.8516/polMal!32!white,0.8516/0.8535/polMal!32!white,0.8535/0.8555/polMal!32!white,0.8555/0.8574/polMal!32!white,0.8574/0.8594/polMal!32!white,0.8594/0.8613/polMal!32!white,0.8613/0.8633/polMal!33!white,0.8633/0.8652/polMal!33!white,0.8652/0.8672/polMal!33!white,0.8672/0.8691/polMal!34!white,0.8691/0.8711/polMal!34!white,0.8711/0.8730/polMal!34!white,0.8730/0.8750/polMal!34!white,0.8750/0.8770/polMal!34!white,0.8770/0.8789/polMal!34!white,0.8789/0.8809/polMal!34!white,0.8809/0.8828/polMal!34!white,0.8828/0.8848/polMal!35!white,0.8848/0.8867/polMal!35!white,0.8867/0.8887/polMal!35!white,0.8887/0.8906/polMal!35!white,0.8906/0.8926/polMal!36!white,0.8926/0.8945/polMal!37!white,0.8945/0.8965/polMal!37!white,0.8965/0.8984/polMal!37!white,0.8984/0.9004/polMal!37!white,0.9004/0.9023/polMal!37!white,0.9023/0.9043/polMal!38!white,0.9043/0.9062/polMal!38!white,0.9062/0.9082/polMal!39!white,0.9082/0.9102/polMal!39!white,0.9102/0.9121/polMal!39!white,0.9121/0.9141/polMal!39!white,0.9141/0.9160/polMal!40!white,0.9160/0.9180/polMal!40!white,0.9180/0.9199/polMal!40!white,0.9199/0.9219/polMal!40!white,0.9219/0.9238/polMal!40!white,0.9238/0.9258/polMal!40!white,0.9258/0.9277/polMal!41!white,0.9277/0.9297/polMal!41!white,0.9297/0.9316/polMal!41!white,0.9316/0.9336/polMal!41!white,0.9336/0.9355/polMal!41!white,0.9355/0.9375/polMal!41!white,0.9375/0.9395/polMal!42!white,0.9395/0.9414/polMal!42!white,0.9414/0.9434/polMal!42!white,0.9434/0.9453/polMal!42!white,0.9453/0.9473/polMal!43!white,0.9473/0.9492/polMal!43!white,0.9492/0.9512/polMal!43!white,0.9512/0.9531/polMal!44!white,0.9531/0.9551/polMal!45!white,0.9551/0.9570/polMal!45!white,0.9570/0.9590/polMal!45!white,0.9590/0.9609/polMal!46!white,0.9609/0.9629/polMal!46!white,0.9629/0.9648/polMal!47!white,0.9648/0.9668/polMal!49!white,0.9668/0.9688/polMal!49!white,0.9688/0.9707/polMal!49!white,0.9707/0.9727/polMal!49!white,0.9727/0.9746/polMal!50!white,0.9746/0.9766/polMal!51!white,0.9766/0.9785/polMal!51!white,0.9785/0.9805/polMal!53!white,0.9805/0.9824/polMal!53!white,0.9824/0.9844/polMal!54!white,0.9844/0.9863/polMal!56!white,0.9863/0.9883/polMal!57!white,0.9883/0.9902/polMal!58!white,0.9902/0.9922/polMal!59!white,0.9922/0.9941/polMal!61!white,0.9941/0.9961/polMal!81!white,0.9961/0.9980/polMal!90!white,0.9980/1.0000/polMal!100!white}
\def\polTIFmissing{0}
\def\polTIFarrows{0.2451/38.91/59.95/polBen,0.4521/24.58/54.27/polBen,0.5205/23.63/37.70/polMal,0.9893/69.53/59.44/polMal}
\def\polTIFhasarrows{1}
\def\polTIFben{38\,$\to$\,51\,\%}
\def\polTIFmal{46\,$\to$\,48\,\%}
\def\polTIFsplit{0.51953}
\def\polTIFn{128}
\def\polTIFev{128}
\def\polTIFC{512}
\def\polTIFstrip{0.0000/0.0020/polBen!100!white,0.0020/0.0039/polBen!99!white,0.0039/0.0059/polBen!98!white,0.0059/0.0078/polBen!98!white,0.0078/0.0098/polBen!97!white,0.0098/0.0117/polBen!95!white,0.0117/0.0137/polBen!95!white,0.0137/0.0156/polBen!95!white,0.0156/0.0176/polBen!94!white,0.0176/0.0195/polBen!94!white,0.0195/0.0215/polBen!93!white,0.0215/0.0234/polBen!92!white,0.0234/0.0254/polBen!91!white,0.0254/0.0273/polBen!91!white,0.0273/0.0293/polBen!91!white,0.0293/0.0312/polBen!91!white,0.0312/0.0332/polBen!91!white,0.0332/0.0352/polBen!90!white,0.0352/0.0371/polBen!90!white,0.0371/0.0391/polBen!89!white,0.0391/0.0410/polBen!89!white,0.0410/0.0430/polBen!88!white,0.0430/0.0449/polBen!88!white,0.0449/0.0469/polBen!88!white,0.0469/0.0488/polBen!88!white,0.0488/0.0508/polBen!87!white,0.0508/0.0527/polBen!87!white,0.0527/0.0547/polBen!87!white,0.0547/0.0566/polBen!87!white,0.0566/0.0586/polBen!87!white,0.0586/0.0605/polBen!86!white,0.0605/0.0625/polBen!86!white,0.0625/0.0645/polBen!85!white,0.0645/0.0664/polBen!85!white,0.0664/0.0684/polBen!85!white,0.0684/0.0703/polBen!85!white,0.0703/0.0723/polBen!85!white,0.0723/0.0742/polBen!84!white,0.0742/0.0762/polBen!84!white,0.0762/0.0781/polBen!84!white,0.0781/0.0801/polBen!83!white,0.0801/0.0820/polBen!83!white,0.0820/0.0840/polBen!83!white,0.0840/0.0859/polBen!83!white,0.0859/0.0879/polBen!83!white,0.0879/0.0898/polBen!83!white,0.0898/0.0918/polBen!83!white,0.0918/0.0938/polBen!83!white,0.0938/0.0957/polBen!83!white,0.0957/0.0977/polBen!83!white,0.0977/0.0996/polBen!83!white,0.0996/0.1016/polBen!83!white,0.1016/0.1035/polBen!82!white,0.1035/0.1055/polBen!82!white,0.1055/0.1074/polBen!82!white,0.1074/0.1094/polBen!82!white,0.1094/0.1113/polBen!82!white,0.1113/0.1133/polBen!82!white,0.1133/0.1152/polBen!82!white,0.1152/0.1172/polBen!82!white,0.1172/0.1191/polBen!82!white,0.1191/0.1211/polBen!82!white,0.1211/0.1230/polBen!81!white,0.1230/0.1250/polBen!81!white,0.1250/0.1270/polBen!81!white,0.1270/0.1289/polBen!81!white,0.1289/0.1309/polBen!81!white,0.1309/0.1328/polBen!81!white,0.1328/0.1348/polBen!81!white,0.1348/0.1367/polBen!81!white,0.1367/0.1387/polBen!80!white,0.1387/0.1406/polBen!80!white,0.1406/0.1426/polBen!80!white,0.1426/0.1445/polBen!80!white,0.1445/0.1465/polBen!80!white,0.1465/0.1484/polBen!80!white,0.1484/0.1504/polBen!80!white,0.1504/0.1523/polBen!80!white,0.1523/0.1543/polBen!79!white,0.1543/0.1562/polBen!79!white,0.1562/0.1582/polBen!79!white,0.1582/0.1602/polBen!79!white,0.1602/0.1621/polBen!79!white,0.1621/0.1641/polBen!79!white,0.1641/0.1660/polBen!79!white,0.1660/0.1680/polBen!79!white,0.1680/0.1699/polBen!79!white,0.1699/0.1719/polBen!79!white,0.1719/0.1738/polBen!78!white,0.1738/0.1758/polBen!78!white,0.1758/0.1777/polBen!78!white,0.1777/0.1797/polBen!78!white,0.1797/0.1816/polBen!77!white,0.1816/0.1836/polBen!77!white,0.1836/0.1855/polBen!77!white,0.1855/0.1875/polBen!77!white,0.1875/0.1895/polBen!77!white,0.1895/0.1914/polBen!77!white,0.1914/0.1934/polBen!77!white,0.1934/0.1953/polBen!77!white,0.1953/0.1973/polBen!77!white,0.1973/0.1992/polBen!77!white,0.1992/0.2012/polBen!76!white,0.2012/0.2031/polBen!76!white,0.2031/0.2051/polBen!76!white,0.2051/0.2070/polBen!76!white,0.2070/0.2090/polBen!76!white,0.2090/0.2109/polBen!76!white,0.2109/0.2129/polBen!76!white,0.2129/0.2148/polBen!76!white,0.2148/0.2168/polBen!76!white,0.2168/0.2188/polBen!76!white,0.2188/0.2207/polBen!76!white,0.2207/0.2227/polBen!76!white,0.2227/0.2246/polBen!76!white,0.2246/0.2266/polBen!76!white,0.2266/0.2285/polBen!76!white,0.2285/0.2305/polBen!76!white,0.2305/0.2324/polBen!76!white,0.2324/0.2344/polBen!76!white,0.2344/0.2363/polBen!76!white,0.2363/0.2383/polBen!75!white,0.2383/0.2402/polBen!75!white,0.2402/0.2422/polBen!75!white,0.2422/0.2441/polBen!75!white,0.2441/0.2461/polBen!75!white,0.2461/0.2480/polBen!75!white,0.2480/0.2500/polBen!74!white,0.2500/0.2520/polBen!74!white,0.2520/0.2539/polBen!74!white,0.2539/0.2559/polBen!74!white,0.2559/0.2578/polBen!74!white,0.2578/0.2598/polBen!74!white,0.2598/0.2617/polBen!73!white,0.2617/0.2637/polBen!73!white,0.2637/0.2656/polBen!73!white,0.2656/0.2676/polBen!73!white,0.2676/0.2695/polBen!73!white,0.2695/0.2715/polBen!73!white,0.2715/0.2734/polBen!73!white,0.2734/0.2754/polBen!73!white,0.2754/0.2773/polBen!73!white,0.2773/0.2793/polBen!73!white,0.2793/0.2812/polBen!73!white,0.2812/0.2832/polBen!73!white,0.2832/0.2852/polBen!73!white,0.2852/0.2871/polBen!72!white,0.2871/0.2891/polBen!72!white,0.2891/0.2910/polBen!72!white,0.2910/0.2930/polBen!72!white,0.2930/0.2949/polBen!72!white,0.2949/0.2969/polBen!72!white,0.2969/0.2988/polBen!72!white,0.2988/0.3008/polBen!72!white,0.3008/0.3027/polBen!72!white,0.3027/0.3047/polBen!71!white,0.3047/0.3066/polBen!71!white,0.3066/0.3086/polBen!70!white,0.3086/0.3105/polBen!70!white,0.3105/0.3125/polBen!70!white,0.3125/0.3145/polBen!70!white,0.3145/0.3164/polBen!70!white,0.3164/0.3184/polBen!70!white,0.3184/0.3203/polBen!70!white,0.3203/0.3223/polBen!70!white,0.3223/0.3242/polBen!70!white,0.3242/0.3262/polBen!69!white,0.3262/0.3281/polBen!69!white,0.3281/0.3301/polBen!69!white,0.3301/0.3320/polBen!69!white,0.3320/0.3340/polBen!69!white,0.3340/0.3359/polBen!69!white,0.3359/0.3379/polBen!69!white,0.3379/0.3398/polBen!69!white,0.3398/0.3418/polBen!69!white,0.3418/0.3438/polBen!69!white,0.3438/0.3457/polBen!68!white,0.3457/0.3477/polBen!68!white,0.3477/0.3496/polBen!67!white,0.3496/0.3516/polBen!67!white,0.3516/0.3535/polBen!67!white,0.3535/0.3555/polBen!67!white,0.3555/0.3574/polBen!67!white,0.3574/0.3594/polBen!67!white,0.3594/0.3613/polBen!66!white,0.3613/0.3633/polBen!66!white,0.3633/0.3652/polBen!66!white,0.3652/0.3672/polBen!66!white,0.3672/0.3691/polBen!66!white,0.3691/0.3711/polBen!66!white,0.3711/0.3730/polBen!66!white,0.3730/0.3750/polBen!65!white,0.3750/0.3770/polBen!65!white,0.3770/0.3789/polBen!65!white,0.3789/0.3809/polBen!65!white,0.3809/0.3828/polBen!65!white,0.3828/0.3848/polBen!65!white,0.3848/0.3867/polBen!65!white,0.3867/0.3887/polBen!64!white,0.3887/0.3906/polBen!64!white,0.3906/0.3926/polBen!64!white,0.3926/0.3945/polBen!64!white,0.3945/0.3965/polBen!64!white,0.3965/0.3984/polBen!64!white,0.3984/0.4004/polBen!64!white,0.4004/0.4023/polBen!64!white,0.4023/0.4043/polBen!64!white,0.4043/0.4062/polBen!64!white,0.4062/0.4082/polBen!63!white,0.4082/0.4102/polBen!63!white,0.4102/0.4121/polBen!63!white,0.4121/0.4141/polBen!63!white,0.4141/0.4160/polBen!63!white,0.4160/0.4180/polBen!63!white,0.4180/0.4199/polBen!63!white,0.4199/0.4219/polBen!62!white,0.4219/0.4238/polBen!62!white,0.4238/0.4258/polBen!62!white,0.4258/0.4277/polBen!61!white,0.4277/0.4297/polBen!61!white,0.4297/0.4316/polBen!61!white,0.4316/0.4336/polBen!61!white,0.4336/0.4355/polBen!61!white,0.4355/0.4375/polBen!61!white,0.4375/0.4395/polBen!61!white,0.4395/0.4414/polBen!61!white,0.4414/0.4434/polBen!60!white,0.4434/0.4453/polBen!60!white,0.4453/0.4473/polBen!60!white,0.4473/0.4492/polBen!60!white,0.4492/0.4512/polBen!60!white,0.4512/0.4531/polBen!59!white,0.4531/0.4551/polBen!59!white,0.4551/0.4570/polBen!59!white,0.4570/0.4590/polBen!59!white,0.4590/0.4609/polBen!59!white,0.4609/0.4629/polBen!59!white,0.4629/0.4648/polBen!58!white,0.4648/0.4668/polBen!58!white,0.4668/0.4688/polBen!58!white,0.4688/0.4707/polBen!58!white,0.4707/0.4727/polBen!58!white,0.4727/0.4746/polBen!57!white,0.4746/0.4766/polBen!57!white,0.4766/0.4785/polBen!56!white,0.4785/0.4805/polBen!55!white,0.4805/0.4824/polBen!55!white,0.4824/0.4844/polBen!54!white,0.4844/0.4863/polBen!54!white,0.4863/0.4883/polBen!54!white,0.4883/0.4902/polBen!54!white,0.4902/0.4922/polBen!53!white,0.4922/0.4941/polBen!53!white,0.4941/0.4961/polBen!52!white,0.4961/0.4980/polBen!52!white,0.4980/0.5000/polBen!49!white,0.5000/0.5020/polBen!47!white,0.5020/0.5039/polBen!47!white,0.5039/0.5059/polBen!47!white,0.5059/0.5078/polBen!46!white,0.5078/0.5098/polBen!45!white,0.5098/0.5117/polBen!45!white,0.5117/0.5137/polBen!45!white,0.5137/0.5156/polBen!44!white,0.5156/0.5176/polBen!42!white,0.5176/0.5195/polBen!35!white,0.5195/0.5215/polMal!53!white,0.5215/0.5234/polMal!53!white,0.5234/0.5254/polMal!55!white,0.5254/0.5273/polMal!55!white,0.5273/0.5293/polMal!57!white,0.5293/0.5312/polMal!59!white,0.5312/0.5332/polMal!59!white,0.5332/0.5352/polMal!59!white,0.5352/0.5371/polMal!60!white,0.5371/0.5391/polMal!61!white,0.5391/0.5410/polMal!61!white,0.5410/0.5430/polMal!61!white,0.5430/0.5449/polMal!62!white,0.5449/0.5469/polMal!62!white,0.5469/0.5488/polMal!62!white,0.5488/0.5508/polMal!62!white,0.5508/0.5527/polMal!63!white,0.5527/0.5547/polMal!63!white,0.5547/0.5566/polMal!64!white,0.5566/0.5586/polMal!64!white,0.5586/0.5605/polMal!64!white,0.5605/0.5625/polMal!64!white,0.5625/0.5645/polMal!65!white,0.5645/0.5664/polMal!66!white,0.5664/0.5684/polMal!66!white,0.5684/0.5703/polMal!66!white,0.5703/0.5723/polMal!66!white,0.5723/0.5742/polMal!66!white,0.5742/0.5762/polMal!66!white,0.5762/0.5781/polMal!66!white,0.5781/0.5801/polMal!66!white,0.5801/0.5820/polMal!66!white,0.5820/0.5840/polMal!66!white,0.5840/0.5859/polMal!67!white,0.5859/0.5879/polMal!67!white,0.5879/0.5898/polMal!67!white,0.5898/0.5918/polMal!67!white,0.5918/0.5938/polMal!67!white,0.5938/0.5957/polMal!67!white,0.5957/0.5977/polMal!67!white,0.5977/0.5996/polMal!68!white,0.5996/0.6016/polMal!68!white,0.6016/0.6035/polMal!69!white,0.6035/0.6055/polMal!69!white,0.6055/0.6074/polMal!69!white,0.6074/0.6094/polMal!70!white,0.6094/0.6113/polMal!70!white,0.6113/0.6133/polMal!70!white,0.6133/0.6152/polMal!70!white,0.6152/0.6172/polMal!70!white,0.6172/0.6191/polMal!70!white,0.6191/0.6211/polMal!70!white,0.6211/0.6230/polMal!70!white,0.6230/0.6250/polMal!70!white,0.6250/0.6270/polMal!71!white,0.6270/0.6289/polMal!71!white,0.6289/0.6309/polMal!71!white,0.6309/0.6328/polMal!71!white,0.6328/0.6348/polMal!72!white,0.6348/0.6367/polMal!72!white,0.6367/0.6387/polMal!72!white,0.6387/0.6406/polMal!72!white,0.6406/0.6426/polMal!72!white,0.6426/0.6445/polMal!72!white,0.6445/0.6465/polMal!73!white,0.6465/0.6484/polMal!73!white,0.6484/0.6504/polMal!73!white,0.6504/0.6523/polMal!73!white,0.6523/0.6543/polMal!73!white,0.6543/0.6562/polMal!73!white,0.6562/0.6582/polMal!73!white,0.6582/0.6602/polMal!74!white,0.6602/0.6621/polMal!74!white,0.6621/0.6641/polMal!74!white,0.6641/0.6660/polMal!74!white,0.6660/0.6680/polMal!74!white,0.6680/0.6699/polMal!74!white,0.6699/0.6719/polMal!74!white,0.6719/0.6738/polMal!74!white,0.6738/0.6758/polMal!74!white,0.6758/0.6777/polMal!75!white,0.6777/0.6797/polMal!75!white,0.6797/0.6816/polMal!75!white,0.6816/0.6836/polMal!75!white,0.6836/0.6855/polMal!75!white,0.6855/0.6875/polMal!75!white,0.6875/0.6895/polMal!75!white,0.6895/0.6914/polMal!75!white,0.6914/0.6934/polMal!75!white,0.6934/0.6953/polMal!75!white,0.6953/0.6973/polMal!75!white,0.6973/0.6992/polMal!75!white,0.6992/0.7012/polMal!75!white,0.7012/0.7031/polMal!76!white,0.7031/0.7051/polMal!76!white,0.7051/0.7070/polMal!76!white,0.7070/0.7090/polMal!76!white,0.7090/0.7109/polMal!77!white,0.7109/0.7129/polMal!77!white,0.7129/0.7148/polMal!77!white,0.7148/0.7168/polMal!77!white,0.7168/0.7188/polMal!77!white,0.7188/0.7207/polMal!77!white,0.7207/0.7227/polMal!77!white,0.7227/0.7246/polMal!77!white,0.7246/0.7266/polMal!77!white,0.7266/0.7285/polMal!77!white,0.7285/0.7305/polMal!77!white,0.7305/0.7324/polMal!77!white,0.7324/0.7344/polMal!77!white,0.7344/0.7363/polMal!77!white,0.7363/0.7383/polMal!77!white,0.7383/0.7402/polMal!78!white,0.7402/0.7422/polMal!78!white,0.7422/0.7441/polMal!78!white,0.7441/0.7461/polMal!78!white,0.7461/0.7480/polMal!78!white,0.7480/0.7500/polMal!78!white,0.7500/0.7520/polMal!78!white,0.7520/0.7539/polMal!78!white,0.7539/0.7559/polMal!79!white,0.7559/0.7578/polMal!79!white,0.7578/0.7598/polMal!79!white,0.7598/0.7617/polMal!79!white,0.7617/0.7637/polMal!79!white,0.7637/0.7656/polMal!79!white,0.7656/0.7676/polMal!79!white,0.7676/0.7695/polMal!79!white,0.7695/0.7715/polMal!79!white,0.7715/0.7734/polMal!79!white,0.7734/0.7754/polMal!79!white,0.7754/0.7773/polMal!79!white,0.7773/0.7793/polMal!79!white,0.7793/0.7812/polMal!79!white,0.7812/0.7832/polMal!79!white,0.7832/0.7852/polMal!79!white,0.7852/0.7871/polMal!79!white,0.7871/0.7891/polMal!80!white,0.7891/0.7910/polMal!80!white,0.7910/0.7930/polMal!80!white,0.7930/0.7949/polMal!80!white,0.7949/0.7969/polMal!80!white,0.7969/0.7988/polMal!80!white,0.7988/0.8008/polMal!81!white,0.8008/0.8027/polMal!81!white,0.8027/0.8047/polMal!81!white,0.8047/0.8066/polMal!81!white,0.8066/0.8086/polMal!81!white,0.8086/0.8105/polMal!81!white,0.8105/0.8125/polMal!81!white,0.8125/0.8145/polMal!81!white,0.8145/0.8164/polMal!81!white,0.8164/0.8184/polMal!82!white,0.8184/0.8203/polMal!82!white,0.8203/0.8223/polMal!83!white,0.8223/0.8242/polMal!83!white,0.8242/0.8262/polMal!83!white,0.8262/0.8281/polMal!83!white,0.8281/0.8301/polMal!83!white,0.8301/0.8320/polMal!83!white,0.8320/0.8340/polMal!83!white,0.8340/0.8359/polMal!83!white,0.8359/0.8379/polMal!83!white,0.8379/0.8398/polMal!83!white,0.8398/0.8418/polMal!83!white,0.8418/0.8438/polMal!83!white,0.8438/0.8457/polMal!83!white,0.8457/0.8477/polMal!83!white,0.8477/0.8496/polMal!83!white,0.8496/0.8516/polMal!84!white,0.8516/0.8535/polMal!84!white,0.8535/0.8555/polMal!84!white,0.8555/0.8574/polMal!84!white,0.8574/0.8594/polMal!85!white,0.8594/0.8613/polMal!85!white,0.8613/0.8633/polMal!85!white,0.8633/0.8652/polMal!85!white,0.8652/0.8672/polMal!85!white,0.8672/0.8691/polMal!85!white,0.8691/0.8711/polMal!85!white,0.8711/0.8730/polMal!85!white,0.8730/0.8750/polMal!85!white,0.8750/0.8770/polMal!85!white,0.8770/0.8789/polMal!85!white,0.8789/0.8809/polMal!85!white,0.8809/0.8828/polMal!85!white,0.8828/0.8848/polMal!85!white,0.8848/0.8867/polMal!85!white,0.8867/0.8887/polMal!86!white,0.8887/0.8906/polMal!86!white,0.8906/0.8926/polMal!86!white,0.8926/0.8945/polMal!86!white,0.8945/0.8965/polMal!86!white,0.8965/0.8984/polMal!86!white,0.8984/0.9004/polMal!87!white,0.9004/0.9023/polMal!87!white,0.9023/0.9043/polMal!87!white,0.9043/0.9062/polMal!87!white,0.9062/0.9082/polMal!87!white,0.9082/0.9102/polMal!87!white,0.9102/0.9121/polMal!87!white,0.9121/0.9141/polMal!87!white,0.9141/0.9160/polMal!88!white,0.9160/0.9180/polMal!88!white,0.9180/0.9199/polMal!88!white,0.9199/0.9219/polMal!88!white,0.9219/0.9238/polMal!88!white,0.9238/0.9258/polMal!88!white,0.9258/0.9277/polMal!88!white,0.9277/0.9297/polMal!89!white,0.9297/0.9316/polMal!89!white,0.9316/0.9336/polMal!89!white,0.9336/0.9355/polMal!89!white,0.9355/0.9375/polMal!89!white,0.9375/0.9395/polMal!90!white,0.9395/0.9414/polMal!91!white,0.9414/0.9434/polMal!91!white,0.9434/0.9453/polMal!91!white,0.9453/0.9473/polMal!92!white,0.9473/0.9492/polMal!92!white,0.9492/0.9512/polMal!92!white,0.9512/0.9531/polMal!92!white,0.9531/0.9551/polMal!92!white,0.9551/0.9570/polMal!92!white,0.9570/0.9590/polMal!92!white,0.9590/0.9609/polMal!92!white,0.9609/0.9629/polMal!92!white,0.9629/0.9648/polMal!93!white,0.9648/0.9668/polMal!93!white,0.9668/0.9688/polMal!93!white,0.9688/0.9707/polMal!93!white,0.9707/0.9727/polMal!94!white,0.9727/0.9746/polMal!94!white,0.9746/0.9766/polMal!96!white,0.9766/0.9785/polMal!96!white,0.9785/0.9805/polMal!96!white,0.9805/0.9824/polMal!96!white,0.9824/0.9844/polMal!96!white,0.9844/0.9863/polMal!96!white,0.9863/0.9883/polMal!96!white,0.9883/0.9902/polMal!96!white,0.9902/0.9922/polMal!97!white,0.9922/0.9941/polMal!97!white,0.9941/0.9961/polMal!98!white,0.9961/0.9980/polMal!98!white,0.9980/1.0000/polMal!100!white}
\def\polDRMDmissing{0}
\def\polDRMDarrows{0.0244/57.07/74.37/polBen,0.1455/6.39/12.24/polBen,0.9580/48.77/26.59/polMal}
\def\polDRMDhasarrows{1}
\def\polDRMDben{17\,$\to$\,22\,\%}
\def\polDRMDmal{13\,$\to$\,8\,\%}
\def\polDRMDsplit{0.28711}
\def\polDRMDn{549}
\def\polDRMDev{549}
\def\polDRMDC{512}
\def\polDRMDstrip{0.0000/0.0020/polBen!100!white,0.0020/0.0039/polBen!98!white,0.0039/0.0059/polBen!97!white,0.0059/0.0078/polBen!94!white,0.0078/0.0098/polBen!93!white,0.0098/0.0117/polBen!93!white,0.0117/0.0137/polBen!91!white,0.0137/0.0156/polBen!88!white,0.0156/0.0176/polBen!86!white,0.0176/0.0195/polBen!85!white,0.0195/0.0215/polBen!82!white,0.0215/0.0234/polBen!82!white,0.0234/0.0254/polBen!79!white,0.0254/0.0273/polBen!74!white,0.0273/0.0293/polBen!73!white,0.0293/0.0312/polBen!73!white,0.0312/0.0332/polBen!72!white,0.0332/0.0352/polBen!70!white,0.0352/0.0371/polBen!69!white,0.0371/0.0391/polBen!68!white,0.0391/0.0410/polBen!68!white,0.0410/0.0430/polBen!67!white,0.0430/0.0449/polBen!67!white,0.0449/0.0469/polBen!66!white,0.0469/0.0488/polBen!65!white,0.0488/0.0508/polBen!65!white,0.0508/0.0527/polBen!64!white,0.0527/0.0547/polBen!63!white,0.0547/0.0566/polBen!62!white,0.0566/0.0586/polBen!61!white,0.0586/0.0605/polBen!59!white,0.0605/0.0625/polBen!59!white,0.0625/0.0645/polBen!58!white,0.0645/0.0664/polBen!57!white,0.0664/0.0684/polBen!56!white,0.0684/0.0703/polBen!56!white,0.0703/0.0723/polBen!55!white,0.0723/0.0742/polBen!55!white,0.0742/0.0762/polBen!50!white,0.0762/0.0781/polBen!49!white,0.0781/0.0801/polBen!49!white,0.0801/0.0820/polBen!49!white,0.0820/0.0840/polBen!49!white,0.0840/0.0859/polBen!48!white,0.0859/0.0879/polBen!46!white,0.0879/0.0898/polBen!46!white,0.0898/0.0918/polBen!44!white,0.0918/0.0938/polBen!43!white,0.0938/0.0957/polBen!43!white,0.0957/0.0977/polBen!42!white,0.0977/0.0996/polBen!42!white,0.0996/0.1016/polBen!41!white,0.1016/0.1035/polBen!41!white,0.1035/0.1055/polBen!41!white,0.1055/0.1074/polBen!40!white,0.1074/0.1094/polBen!39!white,0.1094/0.1113/polBen!36!white,0.1113/0.1133/polBen!36!white,0.1133/0.1152/polBen!36!white,0.1152/0.1172/polBen!36!white,0.1172/0.1191/polBen!35!white,0.1191/0.1211/polBen!34!white,0.1211/0.1230/polBen!34!white,0.1230/0.1250/polBen!33!white,0.1250/0.1270/polBen!33!white,0.1270/0.1289/polBen!32!white,0.1289/0.1309/polBen!32!white,0.1309/0.1328/polBen!32!white,0.1328/0.1348/polBen!31!white,0.1348/0.1367/polBen!30!white,0.1367/0.1387/polBen!29!white,0.1387/0.1406/polBen!27!white,0.1406/0.1426/polBen!27!white,0.1426/0.1445/polBen!27!white,0.1445/0.1465/polBen!27!white,0.1465/0.1484/polBen!25!white,0.1484/0.1504/polBen!25!white,0.1504/0.1523/polBen!24!white,0.1523/0.1543/polBen!24!white,0.1543/0.1562/polBen!24!white,0.1562/0.1582/polBen!24!white,0.1582/0.1602/polBen!23!white,0.1602/0.1621/polBen!23!white,0.1621/0.1641/polBen!23!white,0.1641/0.1660/polBen!22!white,0.1660/0.1680/polBen!22!white,0.1680/0.1699/polBen!21!white,0.1699/0.1719/polBen!21!white,0.1719/0.1738/polBen!21!white,0.1738/0.1758/polBen!20!white,0.1758/0.1777/polBen!20!white,0.1777/0.1797/polBen!20!white,0.1797/0.1816/polBen!20!white,0.1816/0.1836/polBen!19!white,0.1836/0.1855/polBen!19!white,0.1855/0.1875/polBen!19!white,0.1875/0.1895/polBen!19!white,0.1895/0.1914/polBen!19!white,0.1914/0.1934/polBen!18!white,0.1934/0.1953/polBen!18!white,0.1953/0.1973/polBen!16!white,0.1973/0.1992/polBen!16!white,0.1992/0.2012/polBen!16!white,0.2012/0.2031/polBen!16!white,0.2031/0.2051/polBen!15!white,0.2051/0.2070/polBen!15!white,0.2070/0.2090/polBen!14!white,0.2090/0.2109/polBen!13!white,0.2109/0.2129/polBen!13!white,0.2129/0.2148/polBen!13!white,0.2148/0.2168/polBen!13!white,0.2168/0.2188/polBen!13!white,0.2188/0.2207/polBen!13!white,0.2207/0.2227/polBen!13!white,0.2227/0.2246/polBen!12!white,0.2246/0.2266/polBen!12!white,0.2266/0.2285/polBen!11!white,0.2285/0.2305/polBen!11!white,0.2305/0.2324/polBen!11!white,0.2324/0.2344/polBen!10!white,0.2344/0.2363/polBen!10!white,0.2363/0.2383/polBen!10!white,0.2383/0.2402/polBen!10!white,0.2402/0.2422/polBen!9!white,0.2422/0.2441/polBen!9!white,0.2441/0.2461/polBen!9!white,0.2461/0.2480/polBen!9!white,0.2480/0.2500/polBen!8!white,0.2500/0.2520/polBen!8!white,0.2520/0.2539/polBen!6!white,0.2539/0.2559/polBen!6!white,0.2559/0.2578/polBen!6!white,0.2578/0.2598/polBen!6!white,0.2598/0.2617/polBen!4!white,0.2617/0.2637/polBen!4!white,0.2637/0.2656/polBen!4!white,0.2656/0.2676/polBen!0!white,0.2676/0.2695/polBen!0!white,0.2695/0.2715/polBen!0!white,0.2715/0.2734/polBen!0!white,0.2734/0.2754/polBen!0!white,0.2754/0.2773/polBen!0!white,0.2773/0.2793/polBen!0!white,0.2793/0.2812/polBen!0!white,0.2812/0.2832/polBen!0!white,0.2832/0.2852/polBen!0!white,0.2852/0.2871/polBen!0!white,0.2871/0.2891/polMal!0!white,0.2891/0.2910/polMal!0!white,0.2910/0.2930/polMal!0!white,0.2930/0.2949/polMal!0!white,0.2949/0.2969/polMal!0!white,0.2969/0.2988/polMal!0!white,0.2988/0.3008/polMal!0!white,0.3008/0.3027/polMal!0!white,0.3027/0.3047/polMal!0!white,0.3047/0.3066/polMal!0!white,0.3066/0.3086/polMal!0!white,0.3086/0.3105/polMal!0!white,0.3105/0.3125/polMal!0!white,0.3125/0.3145/polMal!0!white,0.3145/0.3164/polMal!0!white,0.3164/0.3184/polMal!0!white,0.3184/0.3203/polMal!0!white,0.3203/0.3223/polMal!0!white,0.3223/0.3242/polMal!0!white,0.3242/0.3262/polMal!0!white,0.3262/0.3281/polMal!0!white,0.3281/0.3301/polMal!0!white,0.3301/0.3320/polMal!0!white,0.3320/0.3340/polMal!5!white,0.3340/0.3359/polMal!5!white,0.3359/0.3379/polMal!5!white,0.3379/0.3398/polMal!5!white,0.3398/0.3418/polMal!5!white,0.3418/0.3438/polMal!5!white,0.3438/0.3457/polMal!5!white,0.3457/0.3477/polMal!5!white,0.3477/0.3496/polMal!5!white,0.3496/0.3516/polMal!5!white,0.3516/0.3535/polMal!5!white,0.3535/0.3555/polMal!5!white,0.3555/0.3574/polMal!5!white,0.3574/0.3594/polMal!5!white,0.3594/0.3613/polMal!5!white,0.3613/0.3633/polMal!5!white,0.3633/0.3652/polMal!5!white,0.3652/0.3672/polMal!7!white,0.3672/0.3691/polMal!7!white,0.3691/0.3711/polMal!7!white,0.3711/0.3730/polMal!7!white,0.3730/0.3750/polMal!7!white,0.3750/0.3770/polMal!7!white,0.3770/0.3789/polMal!7!white,0.3789/0.3809/polMal!7!white,0.3809/0.3828/polMal!8!white,0.3828/0.3848/polMal!8!white,0.3848/0.3867/polMal!8!white,0.3867/0.3887/polMal!8!white,0.3887/0.3906/polMal!8!white,0.3906/0.3926/polMal!8!white,0.3926/0.3945/polMal!8!white,0.3945/0.3965/polMal!8!white,0.3965/0.3984/polMal!8!white,0.3984/0.4004/polMal!8!white,0.4004/0.4023/polMal!8!white,0.4023/0.4043/polMal!8!white,0.4043/0.4062/polMal!10!white,0.4062/0.4082/polMal!10!white,0.4082/0.4102/polMal!10!white,0.4102/0.4121/polMal!10!white,0.4121/0.4141/polMal!10!white,0.4141/0.4160/polMal!10!white,0.4160/0.4180/polMal!10!white,0.4180/0.4199/polMal!10!white,0.4199/0.4219/polMal!10!white,0.4219/0.4238/polMal!11!white,0.4238/0.4258/polMal!12!white,0.4258/0.4277/polMal!12!white,0.4277/0.4297/polMal!12!white,0.4297/0.4316/polMal!13!white,0.4316/0.4336/polMal!13!white,0.4336/0.4355/polMal!13!white,0.4355/0.4375/polMal!13!white,0.4375/0.4395/polMal!13!white,0.4395/0.4414/polMal!13!white,0.4414/0.4434/polMal!13!white,0.4434/0.4453/polMal!13!white,0.4453/0.4473/polMal!13!white,0.4473/0.4492/polMal!13!white,0.4492/0.4512/polMal!13!white,0.4512/0.4531/polMal!13!white,0.4531/0.4551/polMal!14!white,0.4551/0.4570/polMal!14!white,0.4570/0.4590/polMal!14!white,0.4590/0.4609/polMal!14!white,0.4609/0.4629/polMal!14!white,0.4629/0.4648/polMal!15!white,0.4648/0.4668/polMal!15!white,0.4668/0.4688/polMal!16!white,0.4688/0.4707/polMal!16!white,0.4707/0.4727/polMal!16!white,0.4727/0.4746/polMal!16!white,0.4746/0.4766/polMal!16!white,0.4766/0.4785/polMal!16!white,0.4785/0.4805/polMal!16!white,0.4805/0.4824/polMal!16!white,0.4824/0.4844/polMal!16!white,0.4844/0.4863/polMal!16!white,0.4863/0.4883/polMal!17!white,0.4883/0.4902/polMal!17!white,0.4902/0.4922/polMal!17!white,0.4922/0.4941/polMal!17!white,0.4941/0.4961/polMal!17!white,0.4961/0.4980/polMal!17!white,0.4980/0.5000/polMal!18!white,0.5000/0.5020/polMal!18!white,0.5020/0.5039/polMal!19!white,0.5039/0.5059/polMal!20!white,0.5059/0.5078/polMal!20!white,0.5078/0.5098/polMal!20!white,0.5098/0.5117/polMal!20!white,0.5117/0.5137/polMal!20!white,0.5137/0.5156/polMal!20!white,0.5156/0.5176/polMal!21!white,0.5176/0.5195/polMal!21!white,0.5195/0.5215/polMal!21!white,0.5215/0.5234/polMal!21!white,0.5234/0.5254/polMal!22!white,0.5254/0.5273/polMal!22!white,0.5273/0.5293/polMal!22!white,0.5293/0.5312/polMal!22!white,0.5312/0.5332/polMal!22!white,0.5332/0.5352/polMal!22!white,0.5352/0.5371/polMal!22!white,0.5371/0.5391/polMal!23!white,0.5391/0.5410/polMal!23!white,0.5410/0.5430/polMal!23!white,0.5430/0.5449/polMal!23!white,0.5449/0.5469/polMal!23!white,0.5469/0.5488/polMal!23!white,0.5488/0.5508/polMal!23!white,0.5508/0.5527/polMal!23!white,0.5527/0.5547/polMal!24!white,0.5547/0.5566/polMal!24!white,0.5566/0.5586/polMal!24!white,0.5586/0.5605/polMal!24!white,0.5605/0.5625/polMal!24!white,0.5625/0.5645/polMal!24!white,0.5645/0.5664/polMal!24!white,0.5664/0.5684/polMal!25!white,0.5684/0.5703/polMal!25!white,0.5703/0.5723/polMal!25!white,0.5723/0.5742/polMal!25!white,0.5742/0.5762/polMal!26!white,0.5762/0.5781/polMal!26!white,0.5781/0.5801/polMal!26!white,0.5801/0.5820/polMal!26!white,0.5820/0.5840/polMal!26!white,0.5840/0.5859/polMal!27!white,0.5859/0.5879/polMal!27!white,0.5879/0.5898/polMal!27!white,0.5898/0.5918/polMal!27!white,0.5918/0.5938/polMal!27!white,0.5938/0.5957/polMal!27!white,0.5957/0.5977/polMal!28!white,0.5977/0.5996/polMal!28!white,0.5996/0.6016/polMal!28!white,0.6016/0.6035/polMal!28!white,0.6035/0.6055/polMal!29!white,0.6055/0.6074/polMal!29!white,0.6074/0.6094/polMal!29!white,0.6094/0.6113/polMal!29!white,0.6113/0.6133/polMal!29!white,0.6133/0.6152/polMal!30!white,0.6152/0.6172/polMal!30!white,0.6172/0.6191/polMal!30!white,0.6191/0.6211/polMal!30!white,0.6211/0.6230/polMal!30!white,0.6230/0.6250/polMal!30!white,0.6250/0.6270/polMal!30!white,0.6270/0.6289/polMal!30!white,0.6289/0.6309/polMal!30!white,0.6309/0.6328/polMal!31!white,0.6328/0.6348/polMal!31!white,0.6348/0.6367/polMal!31!white,0.6367/0.6387/polMal!31!white,0.6387/0.6406/polMal!32!white,0.6406/0.6426/polMal!32!white,0.6426/0.6445/polMal!32!white,0.6445/0.6465/polMal!32!white,0.6465/0.6484/polMal!32!white,0.6484/0.6504/polMal!32!white,0.6504/0.6523/polMal!33!white,0.6523/0.6543/polMal!33!white,0.6543/0.6562/polMal!34!white,0.6562/0.6582/polMal!34!white,0.6582/0.6602/polMal!34!white,0.6602/0.6621/polMal!34!white,0.6621/0.6641/polMal!34!white,0.6641/0.6660/polMal!34!white,0.6660/0.6680/polMal!34!white,0.6680/0.6699/polMal!35!white,0.6699/0.6719/polMal!35!white,0.6719/0.6738/polMal!35!white,0.6738/0.6758/polMal!35!white,0.6758/0.6777/polMal!35!white,0.6777/0.6797/polMal!35!white,0.6797/0.6816/polMal!35!white,0.6816/0.6836/polMal!35!white,0.6836/0.6855/polMal!35!white,0.6855/0.6875/polMal!35!white,0.6875/0.6895/polMal!36!white,0.6895/0.6914/polMal!36!white,0.6914/0.6934/polMal!36!white,0.6934/0.6953/polMal!36!white,0.6953/0.6973/polMal!36!white,0.6973/0.6992/polMal!36!white,0.6992/0.7012/polMal!36!white,0.7012/0.7031/polMal!37!white,0.7031/0.7051/polMal!37!white,0.7051/0.7070/polMal!37!white,0.7070/0.7090/polMal!37!white,0.7090/0.7109/polMal!37!white,0.7109/0.7129/polMal!37!white,0.7129/0.7148/polMal!37!white,0.7148/0.7168/polMal!37!white,0.7168/0.7188/polMal!37!white,0.7188/0.7207/polMal!38!white,0.7207/0.7227/polMal!38!white,0.7227/0.7246/polMal!38!white,0.7246/0.7266/polMal!38!white,0.7266/0.7285/polMal!38!white,0.7285/0.7305/polMal!38!white,0.7305/0.7324/polMal!38!white,0.7324/0.7344/polMal!39!white,0.7344/0.7363/polMal!39!white,0.7363/0.7383/polMal!39!white,0.7383/0.7402/polMal!39!white,0.7402/0.7422/polMal!39!white,0.7422/0.7441/polMal!39!white,0.7441/0.7461/polMal!39!white,0.7461/0.7480/polMal!39!white,0.7480/0.7500/polMal!39!white,0.7500/0.7520/polMal!40!white,0.7520/0.7539/polMal!40!white,0.7539/0.7559/polMal!40!white,0.7559/0.7578/polMal!40!white,0.7578/0.7598/polMal!40!white,0.7598/0.7617/polMal!40!white,0.7617/0.7637/polMal!41!white,0.7637/0.7656/polMal!41!white,0.7656/0.7676/polMal!41!white,0.7676/0.7695/polMal!41!white,0.7695/0.7715/polMal!41!white,0.7715/0.7734/polMal!41!white,0.7734/0.7754/polMal!42!white,0.7754/0.7773/polMal!42!white,0.7773/0.7793/polMal!42!white,0.7793/0.7812/polMal!42!white,0.7812/0.7832/polMal!42!white,0.7832/0.7852/polMal!42!white,0.7852/0.7871/polMal!42!white,0.7871/0.7891/polMal!42!white,0.7891/0.7910/polMal!43!white,0.7910/0.7930/polMal!43!white,0.7930/0.7949/polMal!43!white,0.7949/0.7969/polMal!43!white,0.7969/0.7988/polMal!43!white,0.7988/0.8008/polMal!43!white,0.8008/0.8027/polMal!44!white,0.8027/0.8047/polMal!44!white,0.8047/0.8066/polMal!45!white,0.8066/0.8086/polMal!45!white,0.8086/0.8105/polMal!45!white,0.8105/0.8125/polMal!45!white,0.8125/0.8145/polMal!46!white,0.8145/0.8164/polMal!46!white,0.8164/0.8184/polMal!47!white,0.8184/0.8203/polMal!47!white,0.8203/0.8223/polMal!47!white,0.8223/0.8242/polMal!47!white,0.8242/0.8262/polMal!47!white,0.8262/0.8281/polMal!47!white,0.8281/0.8301/polMal!47!white,0.8301/0.8320/polMal!47!white,0.8320/0.8340/polMal!48!white,0.8340/0.8359/polMal!48!white,0.8359/0.8379/polMal!48!white,0.8379/0.8398/polMal!48!white,0.8398/0.8418/polMal!49!white,0.8418/0.8438/polMal!49!white,0.8438/0.8457/polMal!49!white,0.8457/0.8477/polMal!49!white,0.8477/0.8496/polMal!51!white,0.8496/0.8516/polMal!51!white,0.8516/0.8535/polMal!52!white,0.8535/0.8555/polMal!52!white,0.8555/0.8574/polMal!52!white,0.8574/0.8594/polMal!52!white,0.8594/0.8613/polMal!52!white,0.8613/0.8633/polMal!53!white,0.8633/0.8652/polMal!53!white,0.8652/0.8672/polMal!53!white,0.8672/0.8691/polMal!54!white,0.8691/0.8711/polMal!54!white,0.8711/0.8730/polMal!54!white,0.8730/0.8750/polMal!54!white,0.8750/0.8770/polMal!54!white,0.8770/0.8789/polMal!55!white,0.8789/0.8809/polMal!55!white,0.8809/0.8828/polMal!55!white,0.8828/0.8848/polMal!55!white,0.8848/0.8867/polMal!55!white,0.8867/0.8887/polMal!55!white,0.8887/0.8906/polMal!55!white,0.8906/0.8926/polMal!55!white,0.8926/0.8945/polMal!56!white,0.8945/0.8965/polMal!56!white,0.8965/0.8984/polMal!56!white,0.8984/0.9004/polMal!57!white,0.9004/0.9023/polMal!58!white,0.9023/0.9043/polMal!58!white,0.9043/0.9062/polMal!58!white,0.9062/0.9082/polMal!58!white,0.9082/0.9102/polMal!59!white,0.9102/0.9121/polMal!59!white,0.9121/0.9141/polMal!59!white,0.9141/0.9160/polMal!59!white,0.9160/0.9180/polMal!60!white,0.9180/0.9199/polMal!61!white,0.9199/0.9219/polMal!61!white,0.9219/0.9238/polMal!61!white,0.9238/0.9258/polMal!61!white,0.9258/0.9277/polMal!62!white,0.9277/0.9297/polMal!62!white,0.9297/0.9316/polMal!62!white,0.9316/0.9336/polMal!62!white,0.9336/0.9355/polMal!63!white,0.9355/0.9375/polMal!64!white,0.9375/0.9395/polMal!65!white,0.9395/0.9414/polMal!66!white,0.9414/0.9434/polMal!68!white,0.9434/0.9453/polMal!69!white,0.9453/0.9473/polMal!71!white,0.9473/0.9492/polMal!71!white,0.9492/0.9512/polMal!71!white,0.9512/0.9531/polMal!72!white,0.9531/0.9551/polMal!73!white,0.9551/0.9570/polMal!73!white,0.9570/0.9590/polMal!77!white,0.9590/0.9609/polMal!81!white,0.9609/0.9629/polMal!82!white,0.9629/0.9648/polMal!83!white,0.9648/0.9668/polMal!83!white,0.9668/0.9688/polMal!86!white,0.9688/0.9707/polMal!86!white,0.9707/0.9727/polMal!87!white,0.9727/0.9746/polMal!87!white,0.9746/0.9766/polMal!88!white,0.9766/0.9785/polMal!88!white,0.9785/0.9805/polMal!88!white,0.9805/0.9824/polMal!88!white,0.9824/0.9844/polMal!89!white,0.9844/0.9863/polMal!91!white,0.9863/0.9883/polMal!93!white,0.9883/0.9902/polMal!94!white,0.9902/0.9922/polMal!97!white,0.9922/0.9941/polMal!98!white,0.9941/0.9961/polMal!98!white,0.9961/0.9980/polMal!99!white,0.9980/1.0000/polMal!100!white}


==> figures/polarity_data/summary.tex <==
\def\polDDmissing{0}
\def\polDDarrows{0.1975/19.57/34.19/polBen,0.4225/5.14/21.47/polBen,0.7375/26.12/11.01/polMal,0.9475/48.38/14.19/polMal}
\def\polDDhasarrows{1}
\def\polDDben{18\,$\to$\,29\,\%}
\def\polDDmal{28\,$\to$\,13\,\%}
\def\polDDsplit{0.52000}
\def\polDDn{109}
\def\polDDev{109}
\def\polDDC{200}
\def\polDDstrip{0.0000/0.0050/polBen!100!white,0.0050/0.0100/polBen!91!white,0.0100/0.0150/polBen!90!white,0.0150/0.0200/polBen!89!white,0.0200/0.0250/polBen!87!white,0.0250/0.0300/polBen!85!white,0.0300/0.0350/polBen!84!white,0.0350/0.0400/polBen!84!white,0.0400/0.0450/polBen!82!white,0.0450/0.0500/polBen!81!white,0.0500/0.0550/polBen!81!white,0.0550/0.0600/polBen!81!white,0.0600/0.0650/polBen!80!white,0.0650/0.0700/polBen!80!white,0.0700/0.0750/polBen!78!white,0.0750/0.0800/polBen!78!white,0.0800/0.0850/polBen!77!white,0.0850/0.0900/polBen!77!white,0.0900/0.0950/polBen!76!white,0.0950/0.1000/polBen!75!white,0.1000/0.1050/polBen!75!white,0.1050/0.1100/polBen!73!white,0.1100/0.1150/polBen!73!white,0.1150/0.1200/polBen!72!white,0.1200/0.1250/polBen!72!white,0.1250/0.1300/polBen!70!white,0.1300/0.1350/polBen!70!white,0.1350/0.1400/polBen!68!white,0.1400/0.1450/polBen!67!white,0.1450/0.1500/polBen!67!white,0.1500/0.1550/polBen!64!white,0.1550/0.1600/polBen!63!white,0.1600/0.1650/polBen!63!white,0.1650/0.1700/polBen!62!white,0.1700/0.1750/polBen!62!white,0.1750/0.1800/polBen!60!white,0.1800/0.1850/polBen!59!white,0.1850/0.1900/polBen!59!white,0.1900/0.1950/polBen!59!white,0.1950/0.2000/polBen!59!white,0.2000/0.2050/polBen!58!white,0.2050/0.2100/polBen!58!white,0.2100/0.2150/polBen!56!white,0.2150/0.2200/polBen!55!white,0.2200/0.2250/polBen!55!white,0.2250/0.2300/polBen!53!white,0.2300/0.2350/polBen!53!white,0.2350/0.2400/polBen!53!white,0.2400/0.2450/polBen!53!white,0.2450/0.2500/polBen!52!white,0.2500/0.2550/polBen!52!white,0.2550/0.2600/polBen!50!white,0.2600/0.2650/polBen!50!white,0.2650/0.2700/polBen!49!white,0.2700/0.2750/polBen!49!white,0.2750/0.2800/polBen!47!white,0.2800/0.2850/polBen!47!white,0.2850/0.2900/polBen!47!white,0.2900/0.2950/polBen!47!white,0.2950/0.3000/polBen!47!white,0.3000/0.3050/polBen!45!white,0.3050/0.3100/polBen!44!white,0.3100/0.3150/polBen!44!white,0.3150/0.3200/polBen!44!white,0.3200/0.3250/polBen!42!white,0.3250/0.3300/polBen!42!white,0.3300/0.3350/polBen!42!white,0.3350/0.3400/polBen!40!white,0.3400/0.3450/polBen!40!white,0.3450/0.3500/polBen!38!white,0.3500/0.3550/polBen!38!white,0.3550/0.3600/polBen!38!white,0.3600/0.3650/polBen!38!white,0.3650/0.3700/polBen!38!white,0.3700/0.3750/polBen!36!white,0.3750/0.3800/polBen!36!white,0.3800/0.3850/polBen!36!white,0.3850/0.3900/polBen!33!white,0.3900/0.3950/polBen!33!white,0.3950/0.4000/polBen!33!white,0.4000/0.4050/polBen!33!white,0.4050/0.4100/polBen!33!white,0.4100/0.4150/polBen!33!white,0.4150/0.4200/polBen!31!white,0.4200/0.4250/polBen!31!white,0.4250/0.4300/polBen!31!white,0.4300/0.4350/polBen!28!white,0.4350/0.4400/polBen!25!white,0.4400/0.4450/polBen!25!white,0.4450/0.4500/polBen!25!white,0.4500/0.4550/polBen!25!white,0.4550/0.4600/polBen!22!white,0.4600/0.4650/polBen!13!white,0.4650/0.4700/polBen!13!white,0.4700/0.4750/polBen!13!white,0.4750/0.4800/polBen!13!white,0.4800/0.4850/polBen!13!white,0.4850/0.4900/polBen!13!white,0.4900/0.4950/polBen!0!white,0.4950/0.5000/polBen!0!white,0.5000/0.5050/polBen!0!white,0.5050/0.5100/polBen!0!white,0.5100/0.5150/polBen!0!white,0.5150/0.5200/polBen!0!white,0.5200/0.5250/polMal!0!white,0.5250/0.5300/polMal!0!white,0.5300/0.5350/polMal!0!white,0.5350/0.5400/polMal!12!white,0.5400/0.5450/polMal!12!white,0.5450/0.5500/polMal!12!white,0.5500/0.5550/polMal!16!white,0.5550/0.5600/polMal!20!white,0.5600/0.5650/polMal!23!white,0.5650/0.5700/polMal!26!white,0.5700/0.5750/polMal!31!white,0.5750/0.5800/polMal!31!white,0.5800/0.5850/polMal!35!white,0.5850/0.5900/polMal!37!white,0.5900/0.5950/polMal!37!white,0.5950/0.6000/polMal!38!white,0.6000/0.6050/polMal!40!white,0.6050/0.6100/polMal!40!white,0.6100/0.6150/polMal!40!white,0.6150/0.6200/polMal!43!white,0.6200/0.6250/polMal!45!white,0.6250/0.6300/polMal!46!white,0.6300/0.6350/polMal!48!white,0.6350/0.6400/polMal!48!white,0.6400/0.6450/polMal!48!white,0.6450/0.6500/polMal!49!white,0.6500/0.6550/polMal!50!white,0.6550/0.6600/polMal!50!white,0.6600/0.6650/polMal!50!white,0.6650/0.6700/polMal!52!white,0.6700/0.6750/polMal!52!white,0.6750/0.6800/polMal!52!white,0.6800/0.6850/polMal!53!white,0.6850/0.6900/polMal!53!white,0.6900/0.6950/polMal!53!white,0.6950/0.7000/polMal!54!white,0.7000/0.7050/polMal!54!white,0.7050/0.7100/polMal!55!white,0.7100/0.7150/polMal!55!white,0.7150/0.7200/polMal!58!white,0.7200/0.7250/polMal!58!white,0.7250/0.7300/polMal!61!white,0.7300/0.7350/polMal!62!white,0.7350/0.7400/polMal!62!white,0.7400/0.7450/polMal!62!white,0.7450/0.7500/polMal!64!white,0.7500/0.7550/polMal!65!white,0.7550/0.7600/polMal!65!white,0.7600/0.7650/polMal!66!white,0.7650/0.7700/polMal!66!white,0.7700/0.7750/polMal!66!white,0.7750/0.7800/polMal!66!white,0.7800/0.7850/polMal!67!white,0.7850/0.7900/polMal!68!white,0.7900/0.7950/polMal!68!white,0.7950/0.8000/polMal!70!white,0.8000/0.8050/polMal!71!white,0.8050/0.8100/polMal!71!white,0.8100/0.8150/polMal!72!white,0.8150/0.8200/polMal!72!white,0.8200/0.8250/polMal!72!white,0.8250/0.8300/polMal!73!white,0.8300/0.8350/polMal!73!white,0.8350/0.8400/polMal!73!white,0.8400/0.8450/polMal!73!white,0.8450/0.8500/polMal!73!white,0.8500/0.8550/polMal!73!white,0.8550/0.8600/polMal!75!white,0.8600/0.8650/polMal!75!white,0.8650/0.8700/polMal!75!white,0.8700/0.8750/polMal!75!white,0.8750/0.8800/polMal!76!white,0.8800/0.8850/polMal!76!white,0.8850/0.8900/polMal!77!white,0.8900/0.8950/polMal!77!white,0.8950/0.9000/polMal!77!white,0.9000/0.9050/polMal!79!white,0.9050/0.9100/polMal!79!white,0.9100/0.9150/polMal!80!white,0.9150/0.9200/polMal!81!white,0.9200/0.9250/polMal!81!white,0.9250/0.9300/polMal!82!white,0.9300/0.9350/polMal!82!white,0.9350/0.9400/polMal!83!white,0.9400/0.9450/polMal!84!white,0.9450/0.9500/polMal!84!white,0.9500/0.9550/polMal!84!white,0.9550/0.9600/polMal!84!white,0.9600/0.9650/polMal!85!white,0.9650/0.9700/polMal!86!white,0.9700/0.9750/polMal!87!white,0.9750/0.9800/polMal!87!white,0.9800/0.9850/polMal!87!white,0.9850/0.9900/polMal!90!white,0.9900/0.9950/polMal!91!white,0.9950/1.0000/polMal!100!white}
\def\polDSFmissing{0}
\def\polDSFarrows{0.2425/80.80/97.97/polBen,0.2725/77.38/97.77/polBen}
\def\polDSFhasarrows{1}
\def\polDSFben{63\,$\to$\,71\,\%}
\def\polDSFmal{unchanged}
\def\polDSFsplit{0.49000}
\def\polDSFn{565}
\def\polDSFev{543}
\def\polDSFC{200}
\def\polDSFstrip{0.0000/0.0050/polBen!100!white,0.0050/0.0100/polBen!100!white,0.0100/0.0150/polBen!99!white,0.0150/0.0200/polBen!99!white,0.0200/0.0250/polBen!99!white,0.0250/0.0300/polBen!99!white,0.0300/0.0350/polBen!99!white,0.0350/0.0400/polBen!99!white,0.0400/0.0450/polBen!98!white,0.0450/0.0500/polBen!98!white,0.0500/0.0550/polBen!98!white,0.0550/0.0600/polBen!98!white,0.0600/0.0650/polBen!98!white,0.0650/0.0700/polBen!98!white,0.0700/0.0750/polBen!98!white,0.0750/0.0800/polBen!98!white,0.0800/0.0850/polBen!98!white,0.0850/0.0900/polBen!98!white,0.0900/0.0950/polBen!98!white,0.0950/0.1000/polBen!98!white,0.1000/0.1050/polBen!98!white,0.1050/0.1100/polBen!98!white,0.1100/0.1150/polBen!98!white,0.1150/0.1200/polBen!97!white,0.1200/0.1250/polBen!97!white,0.1250/0.1300/polBen!97!white,0.1300/0.1350/polBen!97!white,0.1350/0.1400/polBen!97!white,0.1400/0.1450/polBen!97!white,0.1450/0.1500/polBen!97!white,0.1500/0.1550/polBen!96!white,0.1550/0.1600/polBen!96!white,0.1600/0.1650/polBen!96!white,0.1650/0.1700/polBen!95!white,0.1700/0.1750/polBen!95!white,0.1750/0.1800/polBen!95!white,0.1800/0.1850/polBen!95!white,0.1850/0.1900/polBen!94!white,0.1900/0.1950/polBen!94!white,0.1950/0.2000/polBen!94!white,0.2000/0.2050/polBen!93!white,0.2050/0.2100/polBen!93!white,0.2100/0.2150/polBen!93!white,0.2150/0.2200/polBen!93!white,0.2200/0.2250/polBen!92!white,0.2250/0.2300/polBen!92!white,0.2300/0.2350/polBen!92!white,0.2350/0.2400/polBen!91!white,0.2400/0.2450/polBen!91!white,0.2450/0.2500/polBen!90!white,0.2500/0.2550/polBen!90!white,0.2550/0.2600/polBen!90!white,0.2600/0.2650/polBen!90!white,0.2650/0.2700/polBen!89!white,0.2700/0.2750/polBen!89!white,0.2750/0.2800/polBen!89!white,0.2800/0.2850/polBen!88!white,0.2850/0.2900/polBen!88!white,0.2900/0.2950/polBen!88!white,0.2950/0.3000/polBen!88!white,0.3000/0.3050/polBen!88!white,0.3050/0.3100/polBen!86!white,0.3100/0.3150/polBen!86!white,0.3150/0.3200/polBen!85!white,0.3200/0.3250/polBen!85!white,0.3250/0.3300/polBen!83!white,0.3300/0.3350/polBen!83!white,0.3350/0.3400/polBen!82!white,0.3400/0.3450/polBen!80!white,0.3450/0.3500/polBen!79!white,0.3500/0.3550/polBen!76!white,0.3550/0.3600/polBen!63!white,0.3600/0.3650/polBen!52!white,0.3650/0.3700/polBen!42!white,0.3700/0.3750/polBen!21!white,0.3750/0.3800/polBen!11!white,0.3800/0.3850/polBen!0!white,0.3850/0.3900/polBen!0!white,0.3900/0.3950/polBen!0!white,0.3950/0.4000/polBen!0!white,0.4000/0.4050/polBen!0!white,0.4050/0.4100/polBen!0!white,0.4100/0.4150/polBen!0!white,0.4150/0.4200/polBen!0!white,0.4200/0.4250/polBen!0!white,0.4250/0.4300/polBen!0!white,0.4300/0.4350/polBen!0!white,0.4350/0.4400/polBen!0!white,0.4400/0.4450/polBen!0!white,0.4450/0.4500/polBen!0!white,0.4500/0.4550/polBen!0!white,0.4550/0.4600/polBen!0!white,0.4600/0.4650/polBen!0!white,0.4650/0.4700/polBen!0!white,0.4700/0.4750/polBen!0!white,0.4750/0.4800/polBen!0!white,0.4800/0.4850/polBen!0!white,0.4850/0.4900/polBen!0!white,0.4900/0.4950/polMal!0!white,0.4950/0.5000/polMal!0!white,0.5000/0.5050/polMal!0!white,0.5050/0.5100/polMal!0!white,0.5100/0.5150/polMal!0!white,0.5150/0.5200/polMal!0!white,0.5200/0.5250/polMal!0!white,0.5250/0.5300/polMal!0!white,0.5300/0.5350/polMal!0!white,0.5350/0.5400/polMal!0!white,0.5400/0.5450/polMal!0!white,0.5450/0.5500/polMal!0!white,0.5500/0.5550/polMal!0!white,0.5550/0.5600/polMal!0!white,0.5600/0.5650/polMal!0!white,0.5650/0.5700/polMal!0!white,0.5700/0.5750/polMal!0!white,0.5750/0.5800/polMal!0!white,0.5800/0.5850/polMal!0!white,0.5850/0.5900/polMal!0!white,0.5900/0.5950/polMal!0!white,0.5950/0.6000/polMal!0!white,0.6000/0.6050/polMal!0!white,0.6050/0.6100/polMal!0!white,0.6100/0.6150/polMal!0!white,0.6150/0.6200/polMal!0!white,0.6200/0.6250/polMal!0!white,0.6250/0.6300/polMal!0!white,0.6300/0.6350/polMal!0!white,0.6350/0.6400/polMal!0!white,0.6400/0.6450/polMal!0!white,0.6450/0.6500/polMal!0!white,0.6500/0.6550/polMal!0!white,0.6550/0.6600/polMal!0!white,0.6600/0.6650/polMal!0!white,0.6650/0.6700/polMal!0!white,0.6700/0.6750/polMal!0!white,0.6750/0.6800/polMal!4!white,0.6800/0.6850/polMal!19!white,0.6850/0.6900/polMal!24!white,0.6900/0.6950/polMal!25!white,0.6950/0.7000/polMal!26!white,0.7000/0.7050/polMal!30!white,0.7050/0.7100/polMal!37!white,0.7100/0.7150/polMal!40!white,0.7150/0.7200/polMal!56!white,0.7200/0.7250/polMal!56!white,0.7250/0.7300/polMal!59!white,0.7300/0.7350/polMal!60!white,0.7350/0.7400/polMal!62!white,0.7400/0.7450/polMal!64!white,0.7450/0.7500/polMal!65!white,0.7500/0.7550/polMal!65!white,0.7550/0.7600/polMal!69!white,0.7600/0.7650/polMal!76!white,0.7650/0.7700/polMal!76!white,0.7700/0.7750/polMal!78!white,0.7750/0.7800/polMal!79!white,0.7800/0.7850/polMal!80!white,0.7850/0.7900/polMal!85!white,0.7900/0.7950/polMal!87!white,0.7950/0.8000/polMal!88!white,0.8000/0.8050/polMal!88!white,0.8050/0.8100/polMal!88!white,0.8100/0.8150/polMal!89!white,0.8150/0.8200/polMal!90!white,0.8200/0.8250/polMal!90!white,0.8250/0.8300/polMal!90!white,0.8300/0.8350/polMal!90!white,0.8350/0.8400/polMal!91!white,0.8400/0.8450/polMal!92!white,0.8450/0.8500/polMal!92!white,0.8500/0.8550/polMal!93!white,0.8550/0.8600/polMal!94!white,0.8600/0.8650/polMal!95!white,0.8650/0.8700/polMal!96!white,0.8700/0.8750/polMal!97!white,0.8750/0.8800/polMal!98!white,0.8800/0.8850/polMal!98!white,0.8850/0.8900/polMal!99!white,0.8900/0.8950/polMal!99!white,0.8950/0.9000/polMal!99!white,0.9000/0.9050/polMal!99!white,0.9050/0.9100/polMal!99!white,0.9100/0.9150/polMal!99!white,0.9150/0.9200/polMal!99!white,0.9200/0.9250/polMal!100!white,0.9250/0.9300/polMal!100!white,0.9300/0.9350/polMal!100!white,0.9350/0.9400/polMal!100!white,0.9400/0.9450/polMal!100!white,0.9450/0.9500/polMal!100!white,0.9500/0.9550/polMal!100!white,0.9550/0.9600/polMal!100!white,0.9600/0.9650/polMal!100!white,0.9650/0.9700/polMal!100!white,0.9700/0.9750/polMal!100!white,0.9750/0.9800/polMal!100!white,0.9800/0.9850/polMal!100!white,0.9850/0.9900/polMal!100!white,0.9900/0.9950/polMal!100!white,0.9950/1.0000/polMal!100!white}
\def\polDSCmissing{0}
\def\polDSCarrows{}
\def\polDSChasarrows{0}
\def\polDSCben{none}
\def\polDSCmal{unchanged}
\def\polDSCsplit{0.00000}
\def\polDSCn{228}
\def\polDSCev{0}
\def\polDSCC{200}
\def\polDSCstrip{0.0000/0.0050/polMal!0!white,0.0050/0.0100/polMal!0!white,0.0100/0.0150/polMal!0!white,0.0150/0.0200/polMal!0!white,0.0200/0.0250/polMal!0!white,0.0250/0.0300/polMal!0!white,0.0300/0.0350/polMal!0!white,0.0350/0.0400/polMal!0!white,0.0400/0.0450/polMal!0!white,0.0450/0.0500/polMal!0!white,0.0500/0.0550/polMal!0!white,0.0550/0.0600/polMal!0!white,0.0600/0.0650/polMal!0!white,0.0650/0.0700/polMal!0!white,0.0700/0.0750/polMal!0!white,0.0750/0.0800/polMal!0!white,0.0800/0.0850/polMal!0!white,0.0850/0.0900/polMal!13!white,0.0900/0.0950/polMal!19!white,0.0950/0.1000/polMal!33!white,0.1000/0.1050/polMal!35!white,0.1050/0.1100/polMal!36!white,0.1100/0.1150/polMal!39!white,0.1150/0.1200/polMal!41!white,0.1200/0.1250/polMal!43!white,0.1250/0.1300/polMal!44!white,0.1300/0.1350/polMal!47!white,0.1350/0.1400/polMal!48!white,0.1400/0.1450/polMal!50!white,0.1450/0.1500/polMal!52!white,0.1500/0.1550/polMal!52!white,0.1550/0.1600/polMal!52!white,0.1600/0.1650/polMal!53!white,0.1650/0.1700/polMal!53!white,0.1700/0.1750/polMal!53!white,0.1750/0.1800/polMal!53!white,0.1800/0.1850/polMal!55!white,0.1850/0.1900/polMal!57!white,0.1900/0.1950/polMal!57!white,0.1950/0.2000/polMal!58!white,0.2000/0.2050/polMal!61!white,0.2050/0.2100/polMal!62!white,0.2100/0.2150/polMal!62!white,0.2150/0.2200/polMal!63!white,0.2200/0.2250/polMal!65!white,0.2250/0.2300/polMal!67!white,0.2300/0.2350/polMal!68!white,0.2350/0.2400/polMal!69!white,0.2400/0.2450/polMal!71!white,0.2450/0.2500/polMal!78!white,0.2500/0.2550/polMal!80!white,0.2550/0.2600/polMal!81!white,0.2600/0.2650/polMal!83!white,0.2650/0.2700/polMal!84!white,0.2700/0.2750/polMal!84!white,0.2750/0.2800/polMal!86!white,0.2800/0.2850/polMal!86!white,0.2850/0.2900/polMal!87!white,0.2900/0.2950/polMal!87!white,0.2950/0.3000/polMal!87!white,0.3000/0.3050/polMal!87!white,0.3050/0.3100/polMal!88!white,0.3100/0.3150/polMal!88!white,0.3150/0.3200/polMal!89!white,0.3200/0.3250/polMal!89!white,0.3250/0.3300/polMal!89!white,0.3300/0.3350/polMal!89!white,0.3350/0.3400/polMal!90!white,0.3400/0.3450/polMal!91!white,0.3450/0.3500/polMal!91!white,0.3500/0.3550/polMal!91!white,0.3550/0.3600/polMal!91!white,0.3600/0.3650/polMal!91!white,0.3650/0.3700/polMal!91!white,0.3700/0.3750/polMal!91!white,0.3750/0.3800/polMal!91!white,0.3800/0.3850/polMal!91!white,0.3850/0.3900/polMal!91!white,0.3900/0.3950/polMal!92!white,0.3950/0.4000/polMal!92!white,0.4000/0.4050/polMal!92!white,0.4050/0.4100/polMal!92!white,0.4100/0.4150/polMal!92!white,0.4150/0.4200/polMal!92!white,0.4200/0.4250/polMal!92!white,0.4250/0.4300/polMal!93!white,0.4300/0.4350/polMal!93!white,0.4350/0.4400/polMal!93!white,0.4400/0.4450/polMal!93!white,0.4450/0.4500/polMal!93!white,0.4500/0.4550/polMal!93!white,0.4550/0.4600/polMal!94!white,0.4600/0.4650/polMal!94!white,0.4650/0.4700/polMal!94!white,0.4700/0.4750/polMal!94!white,0.4750/0.4800/polMal!94!white,0.4800/0.4850/polMal!94!white,0.4850/0.4900/polMal!94!white,0.4900/0.4950/polMal!94!white,0.4950/0.5000/polMal!94!white,0.5000/0.5050/polMal!94!white,0.5050/0.5100/polMal!94!white,0.5100/0.5150/polMal!95!white,0.5150/0.5200/polMal!95!white,0.5200/0.5250/polMal!95!white,0.5250/0.5300/polMal!95!white,0.5300/0.5350/polMal!95!white,0.5350/0.5400/polMal!95!white,0.5400/0.5450/polMal!95!white,0.5450/0.5500/polMal!96!white,0.5500/0.5550/polMal!96!white,0.5550/0.5600/polMal!96!white,0.5600/0.5650/polMal!96!white,0.5650/0.5700/polMal!97!white,0.5700/0.5750/polMal!97!white,0.5750/0.5800/polMal!97!white,0.5800/0.5850/polMal!98!white,0.5850/0.5900/polMal!98!white,0.5900/0.5950/polMal!98!white,0.5950/0.6000/polMal!98!white,0.6000/0.6050/polMal!98!white,0.6050/0.6100/polMal!98!white,0.6100/0.6150/polMal!99!white,0.6150/0.6200/polMal!99!white,0.6200/0.6250/polMal!99!white,0.6250/0.6300/polMal!99!white,0.6300/0.6350/polMal!99!white,0.6350/0.6400/polMal!99!white,0.6400/0.6450/polMal!99!white,0.6450/0.6500/polMal!100!white,0.6500/0.6550/polMal!100!white,0.6550/0.6600/polMal!100!white,0.6600/0.6650/polMal!100!white,0.6650/0.6700/polMal!100!white,0.6700/0.6750/polMal!100!white,0.6750/0.6800/polMal!100!white,0.6800/0.6850/polMal!100!white,0.6850/0.6900/polMal!100!white,0.6900/0.6950/polMal!100!white,0.6950/0.7000/polMal!100!white,0.7000/0.7050/polMal!100!white,0.7050/0.7100/polMal!100!white,0.7100/0.7150/polMal!100!white,0.7150/0.7200/polMal!100!white,0.7200/0.7250/polMal!100!white,0.7250/0.7300/polMal!100!white,0.7300/0.7350/polMal!100!white,0.7350/0.7400/polMal!100!white,0.7400/0.7450/polMal!100!white,0.7450/0.7500/polMal!100!white,0.7500/0.7550/polMal!100!white,0.7550/0.7600/polMal!100!white,0.7600/0.7650/polMal!100!white,0.7650/0.7700/polMal!100!white,0.7700/0.7750/polMal!100!white,0.7750/0.7800/polMal!100!white,0.7800/0.7850/polMal!100!white,0.7850/0.7900/polMal!100!white,0.7900/0.7950/polMal!100!white,0.7950/0.8000/polMal!100!white,0.8000/0.8050/polMal!100!white,0.8050/0.8100/polMal!100!white,0.8100/0.8150/polMal!100!white,0.8150/0.8200/polMal!100!white,0.8200/0.8250/polMal!100!white,0.8250/0.8300/polMal!100!white,0.8300/0.8350/polMal!100!white,0.8350/0.8400/polMal!100!white,0.8400/0.8450/polMal!100!white,0.8450/0.8500/polMal!100!white,0.8500/0.8550/polMal!100!white,0.8550/0.8600/polMal!100!white,0.8600/0.8650/polMal!100!white,0.8650/0.8700/polMal!100!white,0.8700/0.8750/polMal!100!white,0.8750/0.8800/polMal!100!white,0.8800/0.8850/polMal!100!white,0.8850/0.8900/polMal!100!white,0.8900/0.8950/polMal!100!white,0.8950/0.9000/polMal!100!white,0.9000/0.9050/polMal!100!white,0.9050/0.9100/polMal!100!white,0.9100/0.9150/polMal!100!white,0.9150/0.9200/polMal!100!white,0.9200/0.9250/polMal!100!white,0.9250/0.9300/polMal!100!white,0.9300/0.9350/polMal!100!white,0.9350/0.9400/polMal!100!white,0.9400/0.9450/polMal!100!white,0.9450/0.9500/polMal!100!white,0.9500/0.9550/polMal!100!white,0.9550/0.9600/polMal!100!white,0.9600/0.9650/polMal!100!white,0.9650/0.9700/polMal!100!white,0.9700/0.9750/polMal!100!white,0.9750/0.9800/polMal!100!white,0.9800/0.9850/polMal!100!white,0.9850/0.9900/polMal!100!white,0.9900/0.9950/polMal!100!white,0.9950/1.0000/polMal!100!white}
\def\polDSSmissing{0}
\def\polDSSarrows{0.0825/81.87/98.51/polBen,0.1525/27.59/55.60/polBen,0.6025/10.95/46.35/polMal,0.7025/33.22/67.41/polMal}
\def\polDSShasarrows{1}
\def\polDSSben{50\,$\to$\,64\,\%}
\def\polDSSmal{31\,$\to$\,42\,\%}
\def\polDSSsplit{0.24500}
\def\polDSSn{232}
\def\polDSSev{232}
\def\polDSSC{200}
\def\polDSSstrip{0.0000/0.0050/polBen!100!white,0.0050/0.0100/polBen!100!white,0.0100/0.0150/polBen!100!white,0.0150/0.0200/polBen!100!white,0.0200/0.0250/polBen!100!white,0.0250/0.0300/polBen!100!white,0.0300/0.0350/polBen!100!white,0.0350/0.0400/polBen!100!white,0.0400/0.0450/polBen!100!white,0.0450/0.0500/polBen!98!white,0.0500/0.0550/polBen!96!white,0.0550/0.0600/polBen!96!white,0.0600/0.0650/polBen!95!white,0.0650/0.0700/polBen!95!white,0.0700/0.0750/polBen!94!white,0.0750/0.0800/polBen!92!white,0.0800/0.0850/polBen!89!white,0.0850/0.0900/polBen!88!white,0.0900/0.0950/polBen!87!white,0.0950/0.1000/polBen!87!white,0.1000/0.1050/polBen!86!white,0.1050/0.1100/polBen!86!white,0.1100/0.1150/polBen!84!white,0.1150/0.1200/polBen!83!white,0.1200/0.1250/polBen!80!white,0.1250/0.1300/polBen!80!white,0.1300/0.1350/polBen!79!white,0.1350/0.1400/polBen!70!white,0.1400/0.1450/polBen!58!white,0.1450/0.1500/polBen!57!white,0.1500/0.1550/polBen!56!white,0.1550/0.1600/polBen!26!white,0.1600/0.1650/polBen!0!white,0.1650/0.1700/polBen!0!white,0.1700/0.1750/polBen!0!white,0.1750/0.1800/polBen!0!white,0.1800/0.1850/polBen!0!white,0.1850/0.1900/polBen!0!white,0.1900/0.1950/polBen!0!white,0.1950/0.2000/polBen!0!white,0.2000/0.2050/polBen!0!white,0.2050/0.2100/polBen!0!white,0.2100/0.2150/polBen!0!white,0.2150/0.2200/polBen!0!white,0.2200/0.2250/polBen!0!white,0.2250/0.2300/polBen!0!white,0.2300/0.2350/polBen!0!white,0.2350/0.2400/polBen!0!white,0.2400/0.2450/polBen!0!white,0.2450/0.2500/polMal!0!white,0.2500/0.2550/polMal!0!white,0.2550/0.2600/polMal!0!white,0.2600/0.2650/polMal!0!white,0.2650/0.2700/polMal!0!white,0.2700/0.2750/polMal!0!white,0.2750/0.2800/polMal!0!white,0.2800/0.2850/polMal!0!white,0.2850/0.2900/polMal!0!white,0.2900/0.2950/polMal!0!white,0.2950/0.3000/polMal!0!white,0.3000/0.3050/polMal!0!white,0.3050/0.3100/polMal!0!white,0.3100/0.3150/polMal!0!white,0.3150/0.3200/polMal!0!white,0.3200/0.3250/polMal!0!white,0.3250/0.3300/polMal!0!white,0.3300/0.3350/polMal!0!white,0.3350/0.3400/polMal!0!white,0.3400/0.3450/polMal!0!white,0.3450/0.3500/polMal!0!white,0.3500/0.3550/polMal!0!white,0.3550/0.3600/polMal!0!white,0.3600/0.3650/polMal!0!white,0.3650/0.3700/polMal!0!white,0.3700/0.3750/polMal!0!white,0.3750/0.3800/polMal!0!white,0.3800/0.3850/polMal!0!white,0.3850/0.3900/polMal!0!white,0.3900/0.3950/polMal!0!white,0.3950/0.4000/polMal!0!white,0.4000/0.4050/polMal!0!white,0.4050/0.4100/polMal!0!white,0.4100/0.4150/polMal!0!white,0.4150/0.4200/polMal!0!white,0.4200/0.4250/polMal!0!white,0.4250/0.4300/polMal!0!white,0.4300/0.4350/polMal!0!white,0.4350/0.4400/polMal!0!white,0.4400/0.4450/polMal!0!white,0.4450/0.4500/polMal!0!white,0.4500/0.4550/polMal!0!white,0.4550/0.4600/polMal!0!white,0.4600/0.4650/polMal!0!white,0.4650/0.4700/polMal!0!white,0.4700/0.4750/polMal!0!white,0.4750/0.4800/polMal!0!white,0.4800/0.4850/polMal!0!white,0.4850/0.4900/polMal!0!white,0.4900/0.4950/polMal!0!white,0.4950/0.5000/polMal!0!white,0.5000/0.5050/polMal!0!white,0.5050/0.5100/polMal!0!white,0.5100/0.5150/polMal!0!white,0.5150/0.5200/polMal!0!white,0.5200/0.5250/polMal!0!white,0.5250/0.5300/polMal!9!white,0.5300/0.5350/polMal!9!white,0.5350/0.5400/polMal!11!white,0.5400/0.5450/polMal!11!white,0.5450/0.5500/polMal!13!white,0.5500/0.5550/polMal!15!white,0.5550/0.5600/polMal!15!white,0.5600/0.5650/polMal!15!white,0.5650/0.5700/polMal!20!white,0.5700/0.5750/polMal!20!white,0.5750/0.5800/polMal!21!white,0.5800/0.5850/polMal!22!white,0.5850/0.5900/polMal!23!white,0.5900/0.5950/polMal!31!white,0.5950/0.6000/polMal!33!white,0.6000/0.6050/polMal!36!white,0.6050/0.6100/polMal!37!white,0.6100/0.6150/polMal!37!white,0.6150/0.6200/polMal!39!white,0.6200/0.6250/polMal!39!white,0.6250/0.6300/polMal!39!white,0.6300/0.6350/polMal!40!white,0.6350/0.6400/polMal!44!white,0.6400/0.6450/polMal!45!white,0.6450/0.6500/polMal!46!white,0.6500/0.6550/polMal!48!white,0.6550/0.6600/polMal!49!white,0.6600/0.6650/polMal!50!white,0.6650/0.6700/polMal!51!white,0.6700/0.6750/polMal!52!white,0.6750/0.6800/polMal!53!white,0.6800/0.6850/polMal!53!white,0.6850/0.6900/polMal!53!white,0.6900/0.6950/polMal!53!white,0.6950/0.7000/polMal!53!white,0.7000/0.7050/polMal!55!white,0.7050/0.7100/polMal!57!white,0.7100/0.7150/polMal!58!white,0.7150/0.7200/polMal!62!white,0.7200/0.7250/polMal!64!white,0.7250/0.7300/polMal!64!white,0.7300/0.7350/polMal!65!white,0.7350/0.7400/polMal!69!white,0.7400/0.7450/polMal!69!white,0.7450/0.7500/polMal!71!white,0.7500/0.7550/polMal!72!white,0.7550/0.7600/polMal!72!white,0.7600/0.7650/polMal!72!white,0.7650/0.7700/polMal!73!white,0.7700/0.7750/polMal!73!white,0.7750/0.7800/polMal!73!white,0.7800/0.7850/polMal!75!white,0.7850/0.7900/polMal!76!white,0.7900/0.7950/polMal!77!white,0.7950/0.8000/polMal!78!white,0.8000/0.8050/polMal!78!white,0.8050/0.8100/polMal!81!white,0.8100/0.8150/polMal!81!white,0.8150/0.8200/polMal!81!white,0.8200/0.8250/polMal!81!white,0.8250/0.8300/polMal!82!white,0.8300/0.8350/polMal!83!white,0.8350/0.8400/polMal!83!white,0.8400/0.8450/polMal!83!white,0.8450/0.8500/polMal!83!white,0.8500/0.8550/polMal!84!white,0.8550/0.8600/polMal!84!white,0.8600/0.8650/polMal!85!white,0.8650/0.8700/polMal!85!white,0.8700/0.8750/polMal!85!white,0.8750/0.8800/polMal!85!white,0.8800/0.8850/polMal!85!white,0.8850/0.8900/polMal!85!white,0.8900/0.8950/polMal!86!white,0.8950/0.9000/polMal!86!white,0.9000/0.9050/polMal!86!white,0.9050/0.9100/polMal!87!white,0.9100/0.9150/polMal!89!white,0.9150/0.9200/polMal!90!white,0.9200/0.9250/polMal!91!white,0.9250/0.9300/polMal!92!white,0.9300/0.9350/polMal!93!white,0.9350/0.9400/polMal!93!white,0.9400/0.9450/polMal!93!white,0.9450/0.9500/polMal!93!white,0.9500/0.9550/polMal!97!white,0.9550/0.9600/polMal!97!white,0.9600/0.9650/polMal!98!white,0.9650/0.9700/polMal!98!white,0.9700/0.9750/polMal!100!white,0.9750/0.9800/polMal!100!white,0.9800/0.9850/polMal!100!white,0.9850/0.9900/polMal!100!white,0.9900/0.9950/polMal!100!white,0.9950/1.0000/polMal!100!white}


==> figures/polarity_style.tex <==
\definecolor{polMal}{HTML}{CC3311}
\definecolor{polBen}{HTML}{009E73}
\pgfplotsset{
  polax/.style={
    xmin=0, xmax=1, ymin=0, ymax=100, xtick=\empty, ytick={0,25,50,75,100},
    tick label style={font=\footnotesize}, label style={font=\footnotesize},
    title style={font=\footnotesize, yshift=7pt},
    xlabel style={yshift=-13pt},
    axis line style={black!70}, clip=false, set layers,
    every axis plot/.append style={line join=round},
  },
  polclean/.style={line width=0.9pt, dash pattern=on 2.6pt off 1.8pt},
  polatt/.style={line width=2.6pt, opacity=0.7},
}
\tikzset{poldiff/.style={-{Latex[length=1.6mm, width=1.3mm]}, line width=0.6pt}}
\providecommand{\polBgTint}{30}
\def\polNone{none}\def\polUnch{unchanged}
\newcommand{\polPanel}[2]{%
  \edef\polS{\csname pol#2split\endcsname}%
  \edef\polSt{\csname pol#2strip\endcsname}%
  \pgfplotsextra{\begin{pgfonlayer}{axis background}\foreach \xa/\xb/\cc in \polSt {\fill[\cc!\polBgTint!white] (axis cs:\xa,0) rectangle (axis cs:\xb+0.002,100);}\end{pgfonlayer}}%
  \draw[black!45, densely dotted] (axis cs:\polS,0) -- (axis cs:\polS,100);
  \ifdim\polS pt>0.001pt
    \addplot[polatt, polBen, restrict x to domain=0:\polS] table[x=x, y=att, col sep=comma] {\polData/#1.csv};
  \fi
  \addplot[polatt, polMal, restrict x to domain=\polS:1] table[x=x, y=att, col sep=comma] {\polData/#1.csv};
  \ifdim\polS pt>0.001pt
    \addplot[polclean, polBen!60!black, restrict x to domain=0:\polS] table[x=x, y=clean, col sep=comma] {\polData/#1.csv};
  \fi
  \addplot[polclean, polMal!60!black, restrict x to domain=\polS:1] table[x=x, y=clean, col sep=comma] {\polData/#1.csv};
  \ifnum\csname pol#2hasarrows\endcsname=1
    \edef\polA{\csname pol#2arrows\endcsname}%
    \pgfplotsextra{\foreach \px/\py/\pz/\pc in \polA {\draw[poldiff, \pc!70!black] (axis cs:\px,\py) -- (axis cs:\px,\pz);}}%
  \fi
  \edef\polSt{\csname pol#2strip\endcsname}%
  \pgfplotsextra{\foreach \xa/\xb/\cc in \polSt {\fill[\cc] (axis cs:\xa,-10) rectangle (axis cs:\xb,-4);}}%
  \draw[black!45, line width=0.3pt] (axis cs:0,-10) rectangle (axis cs:1,-4);
  \ifdim\polS pt<0.001pt
  \else
    \node[font=\footnotesize, text=polBen!70!black, anchor=north west, inner sep=1pt] at (axis cs:0,-10) {benign};
  \fi
  \node[font=\footnotesize, text=polMal!70!black, anchor=north east, inner sep=1pt] at (axis cs:1,-10) {malware};
  \expandafter\ifx\csname pol#2ben\endcsname\polNone\else
    \node[font=\footnotesize\bfseries, text=polBen!80!black, anchor=south west, inner sep=1.5pt] at (axis cs:0,100) {\csname pol#2ben\endcsname};
  \fi
  \node[font=\footnotesize\bfseries, text=polMal!80!black, anchor=south east, inner sep=1.5pt] at (axis cs:1,100) {\csname pol#2mal\endcsname};
}
\newcommand{\polLegend}[1]{%
  \node[font=\footnotesize, text=black!75, anchor=north] at ($#1+(0,-0.95)$)
    {\tikz[baseline=-0.5ex]\draw[black!70, line width=0.9pt, dash pattern=on 2.6pt off 1.8pt] (0,0)--(0.5,0); clean \quad
     \tikz[baseline=-0.5ex]\draw[black, line width=2.6pt, opacity=0.7] (0,0)--(0.5,0); attacked (white-box APG, $\beta{=}100$)};}


==> figures/tradeoff_data/pareto_front.tex <==
\def\tfPareto{(38.40,38.40) (43.60,38.40) (43.60,34.07) (48.12,34.07) (48.12,30.29)}

